An analytic performance model for overlapping execution of memory-bound loop kernels on multicore CPUs

Complex applications running on multicore processors show a rich performance phenomenology. The growing number of cores per ccNUMA domain complicates performance analysis of memory-bound code since system noise, load imbalance, or task-based programming models can lead to thread desynchronization. Hence, the simplifying assumption that all cores execute the same loop can not be upheld. Motivated by observations on plain and modified versions of the HPCG benchmark, we construct a performance model of execution of memory-bound loop kernels. It can predict the memory bandwidth share per kernel on a memory contention domain depending on the number of active cores and which other workload the kernel is paired with. The only code features required are the single-thread cache line access frequency per kernel, which is directly related to the single-thread memory bandwidth, and its saturated bandwidth. It can either be measured directly or predicted using the Execution-Cache-Memory (ECM) performance model. The computational intensity of the kernels and the detailed structure of the code is of no significance. We validate our model on Intel Broadwell, Intel Cascade Lake, and AMD Rome processors pairing various streaming and stencil kernels. The error in predicting the bandwidth share per kernel is less than 8%.

==> figures/fig2_STREAMJacobi.tex <==
\begin{tikzpicture}	
	% STREAM
	\node [font=\small] at (4,3){\tikz \draw [fill=OliveGreen!8!white] (3.4,0.6) rectangle (0,0) node[pos=.5,Sepia] {\pmb{$40.7 \%,  \SI{16.7}{\giga\byte\per\second}@$ 1T}};};  
	\node [font=\small] at (7.4,3){\tikz \draw [fill=OliveGreen!12!white] (3.4,0.6) rectangle (0,0) node[pos=.5,Sepia] {\pmb{$75.3 \%,  \SI{30.9}{\giga\byte\per\second}@$ 2T}};}; 
	\node [font=\small] at (10.8,3){\tikz \draw [fill=OliveGreen!16!white] (3.4,0.6) rectangle (0,0) node[pos=.5,Sepia] {\pmb{$93.2 \%,  \SI{38.3}{\giga\byte\per\second}@$ 3T}};};
	\node [font=\small] at (14.2,3){\tikz \draw [fill=OliveGreen!20!white] (3.4,0.6) rectangle (0,0) node[pos=.5,Sepia] {\pmb{$100 \%,  \SI{41.1}{\giga\byte\per\second}@$ 4T}};};
	\node [font=\small] at (17.6,3){\tikz \draw [fill=OliveGreen!24!white] (3.4,0.6) rectangle (0,0) node[pos=.5,Sepia] {\pmb{$100 \%,  \SI{41.1}{\giga\byte\per\second}@$ 5T}};};

	% Jacobi-v1
	\node [font=\small] at (4,2){\tikz \draw [fill=CornflowerBlue!8!white] (3.4,0.6) rectangle (0,0) node[pos=.5] {\pmb{$30 \%,  \SI{12.3}{\giga\byte\per\second}@$ 1T}};};  
	\node [font=\small] at (7.4,2){\tikz \draw [fill=CornflowerBlue!12!white] (3.4,0.6) rectangle (0,0) node[pos=.5] {\pmb{$57.6 \%,  \SI{23.6}{\giga\byte\per\second}@$ 2T}};}; 
	\node [font=\small] at (10.8,2){\tikz \draw [fill=CornflowerBlue!16!white] (3.4,0.6) rectangle (0,0) node[pos=.5] {\pmb{$76.9 \%,  \SI{31.5}{\giga\byte\per\second}@$ 3T}};};
	\node [font=\small] at (14.2,2){\tikz \draw [fill=CornflowerBlue!20!white] (3.4,0.6) rectangle (0,0) node[pos=.5] {\pmb{$89.6 \%,  \SI{36.7}{\giga\byte\per\second}@$ 4T}};};
	\node [font=\small] at (17.6,2){\tikz \draw [fill=CornflowerBlue!24!white] (3.4,0.6) rectangle (0,0) node[pos=.5] {\pmb{$98.1 \%,  \SI{40.2}{\giga\byte\per\second}@$ 5T}};}; 
	
	% Jacobi-v1 + STREAM
	\node [font=\small] at (4,1){\tikz \draw [fill=Apricot!8!white] (3.4,0.6) rectangle (0,0) node[pos=.5,blue] {\pmb{$70.7 \%,  \SI{29}{\giga\byte\per\second}@$ 2T}};};  
	\node [font=\small] at (7.4,1){\tikz \draw [fill=Apricot!12!white] (3.4,0.6) rectangle (0,0) node[pos=.5,blue] {\pmb{$100 \%,  \SI{41}{\giga\byte\per\second}@$ 4T}};}; 
	\node [font=\small] at (10.8,1){\tikz \draw [fill=Apricot!16!white] (3.4,0.6) rectangle (0,0) node[pos=.5,blue] {\pmb{$100 \%,  \SI{41}{\giga\byte\per\second}@$ 6T}};};
	\node [font=\small] at (14.2,1){\tikz \draw [fill=Apricot!20!white] (3.4,0.6) rectangle (0,0) node[pos=.5,blue] {\pmb{$100 \%,  \SI{41}{\giga\byte\per\second}@$ 8T}};};
	\node [font=\small] at (17.6,1){\tikz \draw [fill=Apricot!24!white] (3.4,0.6) rectangle (0,0) node[pos=.5,blue] {\pmb{$100 \%,  \SI{41}{\giga\byte\per\second}@$ 10T}};};
	
	\node [font=\small] at (4,0.5){0\% : 0\%};
	\node [font=\small] at (7.5,0.5){5.29\%$\downarrow$ : 4\%$\uparrow$};
	\node [font=\small] at (11,0.5){6\%$\downarrow$ : 6\%$\uparrow$};
	\node [font=\small] at (14.5,0.5){5\%$\downarrow$ : 5\%$\uparrow$};
	\node [font=\small] at (18,0.5){4.5\%$\downarrow$ : 4.5\%$\uparrow$};
	
	\node [font=\small] at (1.6,3){STREAM}; 
	\node [font=\small] at (1.6,2){Jacobi-v1};
	\node [font=\small] at (1.6,1.28){Jacobi-v1};
	\node [font=\small] at (1.65,1){+};
	\node [font=\small] at (1.6,0.72){STREAM};  
	\draw [thick, Blue,decorate,decoration={brace,amplitude=10pt,mirror},xshift=-20pt,yshift=12pt](3,0.1) -- (6.4,0.1) node[black,midway,yshift=-0.6cm] {\footnotesize Scalable regime};
	\draw [thick, red,decorate,decoration={brace,amplitude=10pt,mirror},xshift=77pt,yshift=12pt](3,0.1) -- (16.6,0.1) node[black,midway,yshift=-0.6cm] {\footnotesize Bottleneck regime};

	% Jacobi-v2
	\node [font=\small] at (4,-0.6){\tikz \draw [fill=CornflowerBlue!8!white] (3.4,0.6) rectangle (0,0) node[pos=.5] {\pmb{$21.9 \%,  \SI{8.99}{\giga\byte\per\second}@$ 1T}};};  
	\node [font=\small] at (7.4,-0.6){\tikz \draw [fill=CornflowerBlue!12!white] (3.4,0.6) rectangle (0,0) node[pos=.5] {\pmb{$47.6 \%,  \SI{19.5}{\giga\byte\per\second}@$ 2T}};}; 
	\node [font=\small] at (10.8,-0.6){\tikz \draw [fill=CornflowerBlue!16!white] (3.4,0.6) rectangle (0,0) node[pos=.5] {\pmb{$65.9 \%,  \SI{27.1}{\giga\byte\per\second}@$ 3T}};};
	\node [font=\small] at (14.2,-0.6){\tikz \draw [fill=CornflowerBlue!20!white] (3.4,0.6) rectangle (0,0) node[pos=.5] {\pmb{$78.8 \%,  \SI{32.4}{\giga\byte\per\second}@$ 4T}};};
	\node [font=\small] at (17.6,-0.6){\tikz \draw [fill=CornflowerBlue!24!white] (3.4,0.6) rectangle (0,0) node[pos=.5] {\pmb{$88.4 \%,  \SI{36.3}{\giga\byte\per\second}@$ 5T}};};
	
	% Jacobi-v2 + STREAM
	\node [font=\small] at (4,-1.6){\tikz \draw [fill=Apricot!8!white] (3.4,0.6) rectangle (0,0) node[pos=.5,blue] {\pmb{$62.6 \%,  \SI{26.7}{\giga\byte\per\second}@$ 2T}};};  
	\node [font=\small] at (7.4,-1.6){\tikz \draw [fill=Apricot!12!white] (3.4,0.6) rectangle (0,0) node[pos=.5,blue] {\pmb{$100 \%,  \SI{41.1}{\giga\byte\per\second}@$ 4T}};}; 
	\node [font=\small] at (10.8,-1.6){\tikz \draw [fill=Apricot!16!white] (3.4,0.6) rectangle (0,0) node[pos=.5,blue] {\pmb{$100 \%,  \SI{41.1}{\giga\byte\per\second}@$ 6T}};};
	\node [font=\small] at (14.2,-1.6){\tikz \draw [fill=Apricot!20!white] (3.4,0.6) rectangle (0,0) node[pos=.5,blue] {\pmb{$100 \%,  \SI{41.1}{\giga\byte\per\second}@$ 8T}};};
	\node [font=\small] at (17.6,-1.6){\tikz \draw [fill=Apricot!24!white] (3.4,0.6) rectangle (0,0) node[pos=.5,blue] {\pmb{$100 \%,  \SI{41.1}{\giga\byte\per\second}@$ 10T}};}; 

	\node [font=\small] at (4,-2.1){0\% : 0\%};
	\node [font=\small] at (7.5,-2.1){0\% : 16.5\%$\uparrow$};
	\node [font=\small] at (11,-2.1){2\%$\downarrow$ : 14.2\%$\uparrow$};
	\node [font=\small] at (14.5,-2.1){2.84\%$\downarrow$ : 4.5\%$\uparrow$};
	\node [font=\small] at (18,-2.1){6\%$\downarrow$ : 5.4\%$\uparrow$};
	
	\node [font=\small] at (1.6,-0.6){Jacobi-v2}; 
	\node [font=\small] at (1.6,-1.32){Jacobi-v2};
	\node [font=\small] at (1.65,-1.6){+};	
	\node [font=\small] at (1.6,-1.88){STREAM};
	\draw [thick, ->] (2.3,-3.1) -- (19.3,-3.1);
	\node [font=\small] at (10.8,-3.6){Pressure over memory bus $P_\mathrm{MEM} [\%],$ Bandwidth $[\si{\giga\byte\per\second}] @$ Threads};  
	\draw [thick, Blue,decorate,decoration={brace,amplitude=10pt,mirror},xshift=-20pt,yshift=12pt](3,-2.5) -- (6.4,-2.5) node[black,midway,yshift=-0.6cm] {\footnotesize Scalable regime};
	\draw [thick, red,decorate,decoration={brace,amplitude=10pt,mirror},xshift=77pt,yshift=12pt](3,-2.5) -- (16.6,-2.5) node[black,midway,yshift=-0.6cm] {\footnotesize Bottleneck regime};	
\end{tikzpicture}


%%5T ==> LC_L2, Jacobi-v2
%%Jacobiv2_nOL
%+----------------------------------------+------------+-----------+
%|           Runtime (RDTSC) [s]          |    56.6891 |   57.0135 |
%|          Runtime unhalted [s]          |    55.6884 |   56.1725 |
%|               Clock [MHz]              |  2200.0215 | 2200.0143 |
%|                   CPI                  |     2.4821 |    2.6350 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  5104.3733 | 5083.9725 |
%|   L2 to L1 load data volume [GBytes]   |   289.3622 |  289.8549 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1018.6048 | 1013.2804 |
%|   L1 to L2 evict data volume [GBytes]  |    57.7438 |   57.7706 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  6122.9781 | 6097.2528 |
%|   L1 to/from L2 data volume [GBytes]   |   347.1059 |  347.6255 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  5082.7288 | 5059.3170 |
%|   L3 to L2 load data volume [GBytes]   |   288.1352 |  288.4492 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |   987.3965 |  991.3017 |
%|   L2 to L3 evict data volume [GBytes]  |    55.9746 |   56.5175 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  6070.1253 | 6050.6186 |
%|   L2 to/from L3 data volume [GBytes]   |   344.1098 |  344.9668 |
%%STREAM_nOL
%+----------------------------------------+------------+-----------+
%|           Runtime (RDTSC) [s]          |    47.3652 |   47.4497 |
%|          Runtime unhalted [s]          |    46.7985 |   46.9259 |
%|               Clock [MHz]              |  2200.0233 | 2200.0143 |
%|                   CPI                  |     6.8372 |    7.1476 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  3074.2126 | 3069.1356 |
%|   L2 to L1 load data volume [GBytes]   |   145.6108 |  145.6295 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1023.7400 | 1022.4373 |
%|   L1 to L2 evict data volume [GBytes]  |    48.4897 |   48.5143 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  4097.9525 | 4091.5730 |
%|   L1 to/from L2 data volume [GBytes]   |   194.1005 |  194.1438 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  3061.4951 | 3055.3590 |
%|   L3 to L2 load data volume [GBytes]   |   145.0084 |  144.9758 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |   996.5655 |  991.4637 |
%|   L2 to L3 evict data volume [GBytes]  |    47.2026 |   47.0446 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  4058.0606 | 4046.8227 |
%|   L2 to/from L3 data volume [GBytes]   |   192.2110 |  192.0204 |
%%Jacobiv2_OLSTREAM 6 % decrease
%Runtime (RDTSC) [s]  60.0579 
%L1 to/from L2 bandwidth [MBytes/s] 5777.5140
%L2 to/from L3 bandwidth [MBytes/s] 5730.7672
%%STREAM_OLJacobiv2 5.38 % increase
%  Runtime (RDTSC) [s] 44.9509 
%  L1 to/from L2 bandwidth [MBytes/s] 4318.6811 
%  L2 to/from L3 bandwidth [MBytes/s] 4266.2090
%
%%4T 
%%Jacobiv2_nOL
%|           Runtime (RDTSC) [s]          |    57.5181 |   57.5474 |
%|          Runtime unhalted [s]          |    56.5794 |   56.6084 |
%|               Clock [MHz]              |  2200.0432 | 2199.9482 |
%|                   CPI                  |     2.1038 |    2.1070 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  6310.2747 | 6309.7442 |
%|   L2 to L1 load data volume [GBytes]   |   362.9551 |  363.1093 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1254.8195 | 1254.8495 |
%|   L1 to L2 evict data volume [GBytes]  |    72.1748 |   72.2133 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  7565.0942 | 7564.5937 |
%|   L1 to/from L2 data volume [GBytes]   |   435.1299 |  435.3226 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  6268.9426 | 6268.6723 |
%|   L3 to L2 load data volume [GBytes]   |   360.5777 |  360.7457 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1239.0605 | 1238.3021 |
%|   L2 to L3 evict data volume [GBytes]  |    71.2684 |   71.2611 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  7508.0030 | 7506.9744 |
%|   L2 to/from L3 data volume [GBytes]   |   431.8461 |  432.0068 |
%%STREAM_nOL
%|           Runtime (RDTSC) [s]          |    47.8626 |   47.4816 |
%|          Runtime unhalted [s]          |    46.4575 |   46.0245 |
%|               Clock [MHz]              |  2200.0389 | 2199.9530 |
%|                   CPI                  |     4.4563 |    4.5440 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  3806.5870 | 3839.1516 |
%|   L2 to L1 load data volume [GBytes]   |   182.1932 |  182.2890 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1265.1277 | 1276.2211 |
%|   L1 to L2 evict data volume [GBytes]  |    60.5523 |   60.5970 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  5071.7147 | 5115.3727 |
%|   L1 to/from L2 data volume [GBytes]   |   242.7455 |  242.8860 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  3775.7655 | 3806.2119 |
%|   L3 to L2 load data volume [GBytes]   |   180.7180 |  180.7250 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1230.8521 | 1239.0415 |
%|   L2 to L3 evict data volume [GBytes]  |    58.9118 |   58.8317 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  5006.6176 | 5045.2534 |
%|   L2 to/from L3 data volume [GBytes]   |   239.6297 |  239.5567 |
%%Jacobiv2_OLSTREAM 2.84% decrease
%Runtime (RDTSC) [s] 58.9298
%L1 to/from L2 bandwidth [MBytes/s] 7355.8343 
%L2 to/from L3 bandwidth [MBytes/s] 7317.6611 
%%STREAM_OLJacobiv2 4.5% increase
%Runtime (RDTSC) [s]		 45.6826 
%L1 to/from L2 bandwidth [MBytes/s]  5311.4853
%L2 to/from L3 bandwidth [MBytes/s]  5246.5003
%
%%3T 
%%Jacobiv2_nOL
%|           Runtime (RDTSC) [s]          |    68.7905 |   68.7218 |
%|          Runtime unhalted [s]          |    67.8491 |   67.8365 |
%|               Clock [MHz]              |  2200.0432 | 2200.0452 |
%|                   CPI                  |     1.9025 |    1.9028 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  7040.5215 | 7048.9463 |
%|   L2 to L1 load data volume [GBytes]   |   484.3206 |  484.4161 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1398.9421 | 1400.4193 |
%|   L1 to L2 evict data volume [GBytes]  |    96.2339 |   96.2393 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  8439.4636 | 8449.3656 |
%|   L1 to/from L2 data volume [GBytes]   |   580.5545 |  580.6554 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  6994.5970 | 7003.6976 |
%|   L3 to L2 load data volume [GBytes]   |   481.1615 |  481.3065 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1391.8574 | 1393.3611 |
%|   L2 to L3 evict data volume [GBytes]  |    95.7465 |   95.7542 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  8386.4543 | 8397.0587 |
%|   L2 to/from L3 data volume [GBytes]   |   576.9080 |  577.0607 |
%%STREAM_nOL
%|           Runtime (RDTSC) [s]          |    48.9059 |   48.4362 |
%|          Runtime unhalted [s]          |    47.3009 |   46.9052 |
%|               Clock [MHz]              |  2200.0384 | 2200.0501 |
%|                   CPI                  |     3.5394 |    3.6014 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  4967.1061 | 5014.8881 |
%|   L2 to L1 load data volume [GBytes]   |   242.9209 |  242.9023 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1651.4935 | 1667.7566 |
%|   L1 to L2 evict data volume [GBytes]  |    80.7678 |   80.7798 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  6618.5996 | 6682.6446 |
%|   L1 to/from L2 data volume [GBytes]   |   323.6887 |  323.6821 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  4901.3904 | 4953.5482 |
%|   L3 to L2 load data volume [GBytes]   |   239.7070 |  239.9312 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1594.9303 | 1613.8769 |
%|   L2 to L3 evict data volume [GBytes]  |    78.0015 |   78.1701 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  6496.3208 | 6567.4251 |
%|   L2 to/from L3 data volume [GBytes]   |   317.7085 |  318.1013 |
%%Jacobiv2_OLSTREAM 2% decrease
%Runtime (RDTSC) [s]  69.8560
%L1 to/from L2 bandwidth [MBytes/s]  8270.7123 
%L2 to/from L3 bandwidth [MBytes/s]  8249.3976
%%STREAM_OLJacobiv2 14.2% increase
%Runtime (RDTSC) [s]  41.9338
%L1 to/from L2 bandwidth [MBytes/s]  7715.6274
%L2 to/from L3 bandwidth [MBytes/s]  7564.6525
%
%
%%2T 
%%Jacobiv2_nOL
%|           Runtime (RDTSC) [s]          |   101.9660 |  102.0033 |
%|          Runtime unhalted [s]          |   100.9359 |  100.9315 |
%|               Clock [MHz]              |  2199.9855 | 2200.0456 |
%|                   CPI                  |     1.8906 |    1.8889 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  7119.3174 | 7117.4482 |
%|   L2 to L1 load data volume [GBytes]   |   725.9283 |  726.0032 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1414.9526 | 1414.1622 |
%|   L1 to L2 evict data volume [GBytes]  |   144.2771 |  144.2492 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  8534.2700 | 8531.6104 |
%|   L1 to/from L2 data volume [GBytes]   |   870.2054 |  870.2524 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  7076.1595 | 7075.0213 |
%|   L3 to L2 load data volume [GBytes]   |   721.5277 |  721.6755 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1409.5014 | 1408.9960 |
%|   L2 to L3 evict data volume [GBytes]  |   143.7212 |  143.7222 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  8485.6609 | 8484.0173 |
%|   L2 to/from L3 data volume [GBytes]   |   865.2489 |  865.3978 |
%%STREAM_nOL
%|           Runtime (RDTSC) [s]          |    54.2152 |   54.2849 |
%|          Runtime unhalted [s]          |    51.7186 |   51.9058 |
%|               Clock [MHz]              |  2199.9778 | 2200.0552 |
%|                   CPI                  |     2.7684 |    2.8075 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  6722.5311 | 6712.3340 |
%|   L2 to L1 load data volume [GBytes]   |   364.4632 |  364.3781 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  2236.4362 | 2230.0695 |
%|   L1 to L2 evict data volume [GBytes]  |   121.2488 |  121.0590 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  8958.9673 | 8942.4035 |
%|   L1 to/from L2 data volume [GBytes]   |   485.7119 |  485.4371 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  6567.1880 | 6568.0946 |
%|   L3 to L2 load data volume [GBytes]   |   356.0412 |  356.5481 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  2139.9507 | 2141.5892 |
%|   L2 to L3 evict data volume [GBytes]  |   116.0178 |  116.2559 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  8707.1388 | 8709.6838 |
%|   L2 to/from L3 data volume [GBytes]   |   472.0590 |  472.8040 |
%%Jacobiv2_OLSTREAM No change
%Runtime (RDTSC) [s] 102.2429
%L1 to/from L2 bandwidth [MBytes/s] 8470.9065
%L2 to/from L3 bandwidth [MBytes/s] 8460.1156 
%%STREAM_OLJacobiv2 % 16.5 % increase
%Runtime (RDTSC) [s] 45.2347
%L1 to/from L2 bandwidth [MBytes/s] 10724.0867
%L2 to/from L3 bandwidth [MBytes/s] 10456.3699 


%%%5T ==> LC_L2, Jacobi-v1
%%%Jacobiv2_nOL
%|           Runtime (RDTSC) [s]          |    43.3527 |   43.3007 |
%|          Runtime unhalted [s]          |    42.6446 |   42.6674 |
%|               Clock [MHz]              |  2199.9621 | 2199.9090 |
%|                   CPI                  |     3.5440 |    3.6893 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  5321.9774 | 5332.1504 |
%|   L2 to L1 load data volume [GBytes]   |   230.7220 |  230.8860 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1332.8991 | 1335.1607 |
%|   L1 to L2 evict data volume [GBytes]  |    57.7847 |   57.8134 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  6654.8765 | 6667.3111 |
%|   L1 to/from L2 data volume [GBytes]   |   288.5067 |  288.6994 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  5289.2516 | 5300.8914 |
%|   L3 to L2 load data volume [GBytes]   |   229.3032 |  229.5324 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1297.1796 | 1302.7773 |
%|   L2 to L3 evict data volume [GBytes]  |    56.2362 |   56.4112 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  6586.4312 | 6603.6687 |
%|   L2 to/from L3 data volume [GBytes]   |   285.5394 |  285.9436 |
%|    System to L3 bandwidth [MBytes/s]   |     nan    |    nan    |
%|    System to L3 data volume [GBytes]   |     nan    |    nan    |
%|    L3 to memory bandwidth [MBytes/s]   |          0 |         0 |
%|    L3 to memory data volume [GBytes]   |          0 |         0 |
%| L3 to/from system bandwidth [MBytes/s] |     nan    |    nan    |
%| L3 to/from system data volume [GBytes] |     nan    |    nan    |
%|    Memory read bandwidth [MBytes/s]    | 27118.0068 |         0 |
%|    Memory read data volume [GBytes]    |  1175.6383 |         0 |
%|    Memory write bandwidth [MBytes/s]   | 13349.6913 |         0 |
%|    Memory write data volume [GBytes]   |   578.7449 |         0 |
%|       Memory bandwidth [MBytes/s]      | 40467.6981 |         0 |
%|       Memory data volume [GBytes]      |  1754.3832 |         0 |
%%%STREAM_nOL
%+----------------------------------------+------------+-----------+
%|           Runtime (RDTSC) [s]          |    47.2885 |   47.4510 |
%|          Runtime unhalted [s]          |    46.7274 |   46.9266 |
%|               Clock [MHz]              |  2199.9633 | 2199.9071 |
%|                   CPI                  |     6.9499 |    7.1534 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  3079.2420 | 3068.9484 |
%|   L2 to L1 load data volume [GBytes]   |   145.6127 |  145.6246 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1025.4006 | 1022.5895 |
%|   L1 to L2 evict data volume [GBytes]  |    48.4897 |   48.5229 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  4104.6426 | 4091.5380 |
%|   L1 to/from L2 data volume [GBytes]   |   194.1024 |  194.1475 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  3066.0830 | 3055.1169 |
%|   L3 to L2 load data volume [GBytes]   |   144.9905 |  144.9683 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |   996.7429 |  990.5020 |
%|   L2 to L3 evict data volume [GBytes]  |    47.1345 |   47.0003 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  4062.8259 | 4045.6189 |
%|   L2 to/from L3 data volume [GBytes]   |   192.1249 |  191.9686 |
%|    System to L3 bandwidth [MBytes/s]   |     nan    |    nan    |
%|    System to L3 data volume [GBytes]   |     nan    |    nan    |
%|    L3 to memory bandwidth [MBytes/s]   |          0 |         0 |
%|    L3 to memory data volume [GBytes]   |          0 |         0 |
%| L3 to/from system bandwidth [MBytes/s] |     nan    |    nan    |
%| L3 to/from system data volume [GBytes] |     nan    |    nan    |
%|    Memory read bandwidth [MBytes/s]    | 30800.1494 |         0 |
%|    Memory read data volume [GBytes]    |  1456.4929 |         0 |
%|    Memory write bandwidth [MBytes/s]   | 10282.4749 |         0 |
%|    Memory write data volume [GBytes]   |   486.2428 |         0 |
%|       Memory bandwidth [MBytes/s]      | 41082.6243 |         0 |
%|       Memory data volume [GBytes]      |  1942.7357 |         0 |
%%%Jacobiv2_OLSTREAM 4.75% decrease
%%Runtime (RDTSC) [s] 45.5166
%%L1 to/from L2 bandwidth [MBytes/s] 6338.5919
%%L2 to/from L3 bandwidth [MBytes/s] 6285.7174 
%%%STREAM_OLJacobiv2 4.37% increase
%%Runtime (RDTSC) [s]  45.3099
%%L1 to/from L2 bandwidth [MBytes/s] 4284.1496 
%%L2 to/from L3 bandwidth [MBytes/s] 4227.8315
%%
%%
%%%4T 
%%%Jacobiv2_nOL
%+----------------------------------------+------------+-----------+
%|           Runtime (RDTSC) [s]          |    43.2371 |   43.2619 |
%|          Runtime unhalted [s]          |    42.5686 |   42.6137 |
%|               Clock [MHz]              |  2200.0230 | 2199.8977 |
%|                   CPI                  |     2.8583 |    2.8793 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  6670.7287 | 6670.9525 |
%|   L2 to L1 load data volume [GBytes]   |   288.4232 |  288.5981 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1669.9880 | 1669.7068 |
%|   L1 to L2 evict data volume [GBytes]  |    72.2055 |   72.2347 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  8340.7167 | 8340.6593 |
%|   L1 to/from L2 data volume [GBytes]   |   360.6287 |  360.8328 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  6596.1129 | 6596.5613 |
%|   L3 to L2 load data volume [GBytes]   |   285.1971 |  285.3798 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1615.8227 | 1617.1317 |
%|   L2 to L3 evict data volume [GBytes]  |    69.8636 |   69.9602 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  8211.9356 | 8213.6931 |
%|   L2 to/from L3 data volume [GBytes]   |   355.0606 |  355.3400 |
%|    System to L3 bandwidth [MBytes/s]   |     nan    |    nan    |
%|    System to L3 data volume [GBytes]   |     nan    |    nan    |
%|    L3 to memory bandwidth [MBytes/s]   |          0 |         0 |
%|    L3 to memory data volume [GBytes]   |          0 |         0 |
%| L3 to/from system bandwidth [MBytes/s] |     nan    |    nan    |
%| L3 to/from system data volume [GBytes] |     nan    |    nan    |
%|    Memory read bandwidth [MBytes/s]    | 26952.8310 |         0 |
%|    Memory read data volume [GBytes]    |  1165.3633 |         0 |
%|    Memory write bandwidth [MBytes/s]   | 13378.3650 |         0 |
%|    Memory write data volume [GBytes]   |   578.4422 |         0 |
%|       Memory bandwidth [MBytes/s]      | 40331.1960 |         0 |
%|       Memory data volume [GBytes]      |  1743.8056 |         0 |
%%%STREAM_nOL
%|           Runtime (RDTSC) [s]          |    47.5558 |   47.4715 |
%|          Runtime unhalted [s]          |    47.0260 |   46.9831 |
%|               Clock [MHz]              |  2200.0239 | 2199.8960 |
%|                   CPI                  |     5.5014 |    5.6768 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  3827.2823 | 3834.5288 |
%|   L2 to L1 load data volume [GBytes]   |   182.0093 |  182.0307 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1274.4654 | 1277.1149 |
%|   L1 to L2 evict data volume [GBytes]  |    60.6082 |   60.6265 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  5101.7477 | 5111.6437 |
%|   L1 to/from L2 data volume [GBytes]   |   242.6174 |  242.6572 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  3808.3134 | 3814.6782 |
%|   L3 to L2 load data volume [GBytes]   |   181.1072 |  181.0884 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1240.2723 | 1238.7251 |
%|   L2 to L3 evict data volume [GBytes]  |    58.9821 |   58.8041 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  5048.5857 | 5053.4034 |
%|   L2 to/from L3 data volume [GBytes]   |   240.0893 |  239.8925 |
%|    System to L3 bandwidth [MBytes/s]   |     nan    |    nan    |
%|    System to L3 data volume [GBytes]   |     nan    |    nan    |
%|    L3 to memory bandwidth [MBytes/s]   |          0 |         0 |
%|    L3 to memory data volume [GBytes]   |          0 |         0 |
%| L3 to/from system bandwidth [MBytes/s] |     nan    |    nan    |
%| L3 to/from system data volume [GBytes] |     nan    |    nan    |
%|    Memory read bandwidth [MBytes/s]    | 30704.4158 |         0 |
%|    Memory read data volume [GBytes]    |  1460.1715 |         0 |
%|    Memory write bandwidth [MBytes/s]   | 10255.0688 |         0 |
%|    Memory write data volume [GBytes]   |   487.6875 |         0 |
%|       Memory bandwidth [MBytes/s]      | 40959.4846 |         0 |
%|       Memory data volume [GBytes]      |  1947.8590 |         0 |
%%%Jacobiv2_OLSTREAM 5.1 % decrease
%%Runtime (RDTSC) [s]  45.5634
%%L1 to/from L2 bandwidth [MBytes/s] 7915.2393
%%L2 to/from L3 bandwidth [MBytes/s] 7817.0931
%%%STREAM_OLJacobiv2 5.1% increase
%%Runtime (RDTSC) [s] 45.2181
%%L1 to/from L2 bandwidth [MBytes/s] 5366.5785
%%L2 to/from L3 bandwidth [MBytes/s] 5292.2249
%%
%%
%%%3T 
%%%Jacobiv2_nOL
%+----------------------------------------+------------+------------+
%|           Runtime (RDTSC) [s]          |    44.5123 |    44.3074 |
%|          Runtime unhalted [s]          |    43.8507 |    43.7180 |
%|               Clock [MHz]              |  2200.0184 |  2200.0137 |
%|                   CPI                  |     2.2043 |     2.2643 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  8644.4359 |  8688.5207 |
%|   L2 to L1 load data volume [GBytes]   |   384.7836 |   384.9658 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  2163.9202 |  2173.3168 |
%|   L1 to L2 evict data volume [GBytes]  |    96.3210 |    96.2940 |
%|   L1 to/from L2 bandwidth [MBytes/s]   | 10808.3562 | 10861.8374 |
%|   L1 to/from L2 data volume [GBytes]   |   481.1046 |   481.2598 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  8470.6397 |  8524.2530 |
%|   L3 to L2 load data volume [GBytes]   |   377.0475 |   377.6875 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  2068.4140 |  2083.8906 |
%|   L2 to L3 evict data volume [GBytes]  |    92.0698 |    92.3318 |
%|   L2 to/from L3 bandwidth [MBytes/s]   | 10539.0538 | 10608.1437 |
%|   L2 to/from L3 data volume [GBytes]   |   469.1173 |   470.0193 |
%|    System to L3 bandwidth [MBytes/s]   |     nan    |     nan    |
%|    System to L3 data volume [GBytes]   |     nan    |     nan    |
%|    L3 to memory bandwidth [MBytes/s]   |          0 |          0 |
%|    L3 to memory data volume [GBytes]   |          0 |          0 |
%| L3 to/from system bandwidth [MBytes/s] |     nan    |     nan    |
%| L3 to/from system data volume [GBytes] |     nan    |     nan    |
%|    Memory read bandwidth [MBytes/s]    | 26129.0348 |          0 |
%|    Memory read data volume [GBytes]    |  1163.0629 |          0 |
%|    Memory write bandwidth [MBytes/s]   | 13011.3445 |          0 |
%|    Memory write data volume [GBytes]   |   579.1646 |          0 |
%|       Memory bandwidth [MBytes/s]      | 39140.3792 |          0 |
%|       Memory data volume [GBytes]      |  1742.2275 |          0 |
%+----------------------------------------+------------+------------+
%%%STREAM_nOL
%+----------------------------------------+------------+-----------+
%|           Runtime (RDTSC) [s]          |    47.3418 |   47.4110 |
%|          Runtime unhalted [s]          |    46.7939 |   46.9291 |
%|               Clock [MHz]              |  2200.0172 | 2200.0127 |
%|                   CPI                  |     4.1106 |    4.3014 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  5126.0039 | 5118.7508 |
%|   L2 to L1 load data volume [GBytes]   |   242.6740 |  242.6850 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1707.5968 | 1704.3060 |
%|   L1 to L2 evict data volume [GBytes]  |    80.8406 |   80.8028 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  6833.6008 | 6823.0568 |
%|   L1 to/from L2 data volume [GBytes]   |   323.5147 |  323.4878 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  5072.8429 | 5071.1453 |
%|   L3 to L2 load data volume [GBytes]   |   240.1573 |  240.4280 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1649.8030 | 1649.3881 |
%|   L2 to L3 evict data volume [GBytes]  |    78.1046 |   78.1991 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  6722.6459 | 6720.5333 |
%|   L2 to/from L3 data volume [GBytes]   |   318.2619 |  318.6271 |
%|    System to L3 bandwidth [MBytes/s]   |     nan    |    nan    |
%|    System to L3 data volume [GBytes]   |     nan    |    nan    |
%|    L3 to memory bandwidth [MBytes/s]   |          0 |         0 |
%|    L3 to memory data volume [GBytes]   |          0 |         0 |
%| L3 to/from system bandwidth [MBytes/s] |     nan    |    nan    |
%| L3 to/from system data volume [GBytes] |     nan    |    nan    |
%|    Memory read bandwidth [MBytes/s]    | 30786.8125 |         0 |
%|    Memory read data volume [GBytes]    |  1457.5019 |         0 |
%|    Memory write bandwidth [MBytes/s]   | 10280.9271 |         0 |
%|    Memory write data volume [GBytes]   |   486.7172 |         0 |
%|       Memory bandwidth [MBytes/s]      | 41067.7396 |         0 |
%|       Memory data volume [GBytes]      |  1944.2191 |         0 |
%%%Jacobiv2_OLSTREAM 
%%Runtime (RDTSC) [s] 5.88 decrease  
%%L1 to/from L2 bandwidth [MBytes/s] 10171.8941
%%L2 to/from L3 bandwidth [MBytes/s] 9955.2781
%%%STREAM_OLJacobiv2 6.1 increase
%%Runtime (RDTSC) [s]  44.6081
%%L1 to/from L2 bandwidth [MBytes/s] 7252.8323
%%L2 to/from L3 bandwidth [MBytes/s] 7112.9045
%%
%%
%%%2T 
%%%Jacobiv2_nOL
%+----------------------------------------+------------+------------+
%|           Runtime (RDTSC) [s]          |    50.4988 |    50.4720 |
%|          Runtime unhalted [s]          |    49.9260 |    49.9244 |
%|               Clock [MHz]              |  2199.9703 |  2200.0199 |
%|                   CPI                  |     1.7187 |     1.7335 |
%|   L2 to L1 load bandwidth [MBytes/s]   | 11424.5206 | 11435.0978 |
%|   L2 to L1 load data volume [GBytes]   |   576.9244 |   577.1523 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  2858.9909 |  2859.7572 |
%|   L1 to L2 evict data volume [GBytes]  |   144.3756 |   144.3377 |
%|   L1 to/from L2 bandwidth [MBytes/s]   | 14283.5115 | 14294.8550 |
%|   L1 to/from L2 data volume [GBytes]   |   721.2999 |   721.4899 |
%|   L3 to L2 load bandwidth [MBytes/s]   | 11112.2336 | 11134.6014 |
%|   L3 to L2 load data volume [GBytes]   |   561.1542 |   561.9856 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  2718.4663 |  2722.6895 |
%|   L2 to L3 evict data volume [GBytes]  |   137.2792 |   137.4196 |
%|   L2 to/from L3 bandwidth [MBytes/s]   | 13830.6999 | 13857.2909 |
%|   L2 to/from L3 data volume [GBytes]   |   698.4335 |   699.4052 |
%|    System to L3 bandwidth [MBytes/s]   |     nan    |     nan    |
%|    System to L3 data volume [GBytes]   |     nan    |     nan    |
%|    L3 to memory bandwidth [MBytes/s]   |          0 |          0 |
%|    L3 to memory data volume [GBytes]   |          0 |          0 |
%| L3 to/from system bandwidth [MBytes/s] |     nan    |     nan    |
%| L3 to/from system data volume [GBytes] |     nan    |     nan    |
%|    Memory read bandwidth [MBytes/s]    | 22955.7565 |          0 |
%|    Memory read data volume [GBytes]    |  1159.2377 |          0 |
%|    Memory write bandwidth [MBytes/s]   | 11463.3296 |          0 |
%|    Memory write data volume [GBytes]   |   578.8842 |          0 |
%|       Memory bandwidth [MBytes/s]      | 34419.0861 |          0 |
%|       Memory data volume [GBytes]      |  1738.1219 |          0 |
%%%STREAM_nOL
%|           Runtime (RDTSC) [s]          |    51.2897 |   51.3255 |
%|          Runtime unhalted [s]          |    50.7362 |   50.8311 |
%|               Clock [MHz]              |  2199.9684 | 2200.0199 |
%|                   CPI                  |     3.0303 |    3.1076 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  7095.6596 | 7090.9856 |
%|   L2 to L1 load data volume [GBytes]   |   363.9345 |  363.9481 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  2363.8635 | 2361.4298 |
%|   L1 to L2 evict data volume [GBytes]  |   121.2419 |  121.2015 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  9459.5231 | 9452.4154 |
%|   L1 to/from L2 data volume [GBytes]   |   485.1764 |  485.1496 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  6940.2894 | 6952.3977 |
%|   L3 to L2 load data volume [GBytes]   |   355.9656 |  356.8350 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  2258.0714 | 2264.9388 |
%|   L2 to L3 evict data volume [GBytes]  |   115.8159 |  116.2490 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  9198.3608 | 9217.3364 |
%|   L2 to/from L3 data volume [GBytes]   |   471.7814 |  473.0840 |
%|    System to L3 bandwidth [MBytes/s]   |     nan    |    nan    |
%|    System to L3 data volume [GBytes]   |     nan    |    nan    |
%|    L3 to memory bandwidth [MBytes/s]   |          0 |         0 |
%|    L3 to memory data volume [GBytes]   |          0 |         0 |
%| L3 to/from system bandwidth [MBytes/s] |     nan    |    nan    |
%| L3 to/from system data volume [GBytes] |     nan    |    nan    |
%|    Memory read bandwidth [MBytes/s]    | 28410.5744 |         0 |
%|    Memory read data volume [GBytes]    |  1457.1707 |         0 |
%|    Memory write bandwidth [MBytes/s]   |  9491.5632 |         0 |
%|    Memory write data volume [GBytes]   |   486.8197 |         0 |
%|       Memory bandwidth [MBytes/s]      | 37902.1375 |         0 |
%|       Memory data volume [GBytes]      |  1943.9904 |         0 |
%%%Jacobiv2_OLSTREAM  5.29% decrease
%%Runtime (RDTSC) [s] 53.3231 
%%L1 to/from L2 bandwidth [MBytes/s] 13526.5793
%%L2 to/from L3 bandwidth [MBytes/s] 13114.7386
%%%STREAM_OLJacobiv2  4% increase
%%Runtime (RDTSC) [s] 49.3297
%%L1 to/from L2 bandwidth [MBytes/s] 9835.1831
%%L2 to/from L3 bandwidth [MBytes/s] 9581.6789

%5T 
%ADD_nOL
%|           Runtime (RDTSC) [s]          |    48.3634 |   48.4633 |
%|          Runtime unhalted [s]          |    47.3433 |   47.4886 |
%|               Clock [MHz]              |  2199.9777 | 2199.9758 |
%|                   CPI                  |     7.8913 |    8.1320 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  3011.9304 | 3005.9067 |
%|   L2 to L1 load data volume [GBytes]   |   145.6671 |  145.6762 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1003.0362 | 1001.6669 |
%|   L1 to L2 evict data volume [GBytes]  |    48.5102 |   48.5441 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  4014.9666 | 4007.5736 |
%|   L1 to/from L2 data volume [GBytes]   |   194.1773 |  194.2202 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  2999.7016 | 2992.9848 |
%|   L3 to L2 load data volume [GBytes]   |   145.0756 |  145.0499 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |   977.2723 |  972.0580 |
%|   L2 to L3 evict data volume [GBytes]  |    47.2642 |   47.1091 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  3976.9739 | 3965.0428 |
%|   L2 to/from L3 data volume [GBytes]   |   192.3398 |  192.1591 |
%WAXBPY_nOL
%|           Runtime (RDTSC) [s]          |    47.0332 |   47.0343 |
%|          Runtime unhalted [s]          |    46.4165 |   46.4648 |
%|               Clock [MHz]              |  2199.9756 | 2199.9737 |
%|                   CPI                  |     5.7955 |    5.9296 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  3095.8645 | 3096.2031 |
%|   L2 to L1 load data volume [GBytes]   |   145.6083 |  145.6278 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1030.9172 | 1031.7483 |
%|   L1 to L2 evict data volume [GBytes]  |    48.4873 |   48.5276 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  4126.7816 | 4127.9514 |
%|   L1 to/from L2 data volume [GBytes]   |   194.0956 |  194.1554 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  3082.6068 | 3082.0708 |
%|   L3 to L2 load data volume [GBytes]   |   144.9848 |  144.9631 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1001.2794 |  998.9974 |
%|   L2 to L3 evict data volume [GBytes]  |    47.0933 |   46.9872 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  4083.8862 | 4081.0682 |
%|   L2 to/from L3 data volume [GBytes]   |   192.0781 |  191.9503 |
%ADD_OLWAXPBY
%|           Runtime (RDTSC) [s]          |   48.2911 |  47.4438
%|          Runtime unhalted [s]          |   47.1969 |
%|               Clock [MHz]              | 2199.9820 |
%|                   CPI                  |    8.1136 |
%|   L2 to L1 load bandwidth [MBytes/s]   | 3016.5126 |
%|   L2 to L1 load data volume [GBytes]   |  145.6706 |
%|   L1 to L2 evict bandwidth [MBytes/s]  | 1004.3281 |
%|   L1 to L2 evict data volume [GBytes]  |   48.5001 |
%|   L1 to/from L2 bandwidth [MBytes/s]   | 4020.8408 |4093.3766 
%|   L1 to/from L2 data volume [GBytes]   |  194.1707 |
%|   L3 to L2 load bandwidth [MBytes/s]   | 3003.2199 |
%|   L3 to L2 load data volume [GBytes]   |  145.0287 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  977.1055 |
%|   L2 to L3 evict data volume [GBytes]  |   47.1855 |
%|   L2 to/from L3 bandwidth [MBytes/s]   | 3980.3254 | 4051.3693 
%|   L2 to/from L3 data volume [GBytes]   |  192.2141 |
%WAXPBY_OLADD (8.7% decrease)
%+----------------------------------------+------------+
%|           Runtime (RDTSC) [s]          |    51.1782 | 
%|          Runtime unhalted [s]          |    49.9828 |  
%|               Clock [MHz]              |  2199.9717 | 
%|                   CPI                  |     5.3710 |   
%|   L2 to L1 load bandwidth [MBytes/s]   |  2846.8359 | 
%|   L2 to L1 load data volume [GBytes]   |   145.6959 |  
%|   L1 to L2 evict bandwidth [MBytes/s]  |   948.2850 | 
%|   L1 to L2 evict data volume [GBytes]  |    48.5315 |  
%|   L1 to/from L2 bandwidth [MBytes/s]   |  3795.1209 | 
%|   L1 to/from L2 data volume [GBytes]   |   194.2275 |  
%|   L3 to L2 load bandwidth [MBytes/s]   |  2833.8929 | 
%|   L3 to L2 load data volume [GBytes]   |   145.0335 |  
%|   L2 to L3 evict bandwidth [MBytes/s]  |   917.6542 |  
%|   L2 to L3 evict data volume [GBytes]  |    46.9639 |  
%|   L2 to/from L3 bandwidth [MBytes/s]   |  3751.5471 | 
%|   L2 to/from L3 data volume [GBytes]   |   191.9974 |
%
%4T
%ADD_nOL
%+----------------------------------------+------------+-----------+
%|           Runtime (RDTSC) [s]          |    48.2482 |   48.1758 |
%|          Runtime unhalted [s]          |    47.3896 |   47.3246 |
%|               Clock [MHz]              |  2199.9073 | 2199.9794 |
%|                   CPI                  |     6.5466 |    6.5660 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  3772.9616 | 3778.6546 |
%|   L2 to L1 load data volume [GBytes]   |   182.0387 |  182.0397 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1257.3047 | 1258.2719 |
%|   L1 to L2 evict data volume [GBytes]  |    60.6627 |   60.6183 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  5030.2663 | 5036.9264 |
%|   L1 to/from L2 data volume [GBytes]   |   242.7014 |  242.6580 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  3755.7639 | 3761.5877 |
%|   L3 to L2 load data volume [GBytes]   |   181.2090 |  181.2175 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1224.8471 | 1227.9961 |
%|   L2 to L3 evict data volume [GBytes]  |    59.0967 |   59.1597 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  4980.6110 | 4989.5838 |
%|   L2 to/from L3 data volume [GBytes]   |   240.3057 |  240.3772 |
%WAXBPY_nOL
%+----------------------------------------+------------+-----------+
%|           Runtime (RDTSC) [s]          |    47.3807 |   47.4297 |
%|          Runtime unhalted [s]          |    46.8494 |   46.8851 |
%|               Clock [MHz]              |  2199.9073 | 2199.9773 |
%|                   CPI                  |     4.7700 |    4.7304 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  3841.8179 | 3837.8823 |
%|   L2 to L1 load data volume [GBytes]   |   182.0279 |  182.0298 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1280.0255 | 1277.7826 |
%|   L1 to L2 evict data volume [GBytes]  |    60.6485 |   60.6049 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  5121.8434 | 5115.6649 |
%|   L1 to/from L2 data volume [GBytes]   |   242.6764 |  242.6347 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  3821.5092 | 3817.4300 |
%|   L3 to L2 load data volume [GBytes]   |   181.0657 |  181.0597 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1242.1866 | 1241.7809 |
%|   L2 to L3 evict data volume [GBytes]  |    58.8556 |   58.8973 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  5063.6958 | 5059.2109 |
%|   L2 to/from L3 data volume [GBytes]   |   239.9213 |  239.9571 |
%ADD_OLWAXPBY
%|           Runtime (RDTSC) [s]          |   46.7153 |
%|          Runtime unhalted [s]          |   45.9130 |
%|               Clock [MHz]              | 2199.8385 |
%|                   CPI                  |    6.3887 |
%|   L2 to L1 load bandwidth [MBytes/s]   | 3896.8405 |
%|   L2 to L1 load data volume [GBytes]   |  182.0421 |
%|   L1 to L2 evict bandwidth [MBytes/s]  | 1298.2916 |
%|   L1 to L2 evict data volume [GBytes]  |   60.6501 |
%|   L1 to/from L2 bandwidth [MBytes/s]   | 5195.1321 |
%|   L1 to/from L2 data volume [GBytes]   |  242.6922 |
%|   L3 to L2 load bandwidth [MBytes/s]   | 3876.4015 |
%|   L3 to L2 load data volume [GBytes]   |  181.0873 |
%|   L2 to L3 evict bandwidth [MBytes/s]  | 1264.0277 |
%|   L2 to L3 evict data volume [GBytes]  |   59.0494 |
%|   L2 to/from L3 bandwidth [MBytes/s]   | 5140.4292 |
%|   L2 to/from L3 data volume [GBytes]   |  240.1367 |
%WAXPBY_OLADD (3.2 % decrease)
%|           Runtime (RDTSC) [s]          |    48.9804 |   
%|          Runtime unhalted [s]          |    47.9730 |   
%|               Clock [MHz]              |  2199.9671 | 
%|                   CPI                  |     4.4598 |   
%|   L2 to L1 load bandwidth [MBytes/s]   |  3717.3682 | 
%|   L2 to L1 load data volume [GBytes]   |   182.0781 |  
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1238.3164 | 
%|   L1 to L2 evict data volume [GBytes]  |    60.6532 | 
%|   L1 to/from L2 bandwidth [MBytes/s]   |  4955.6846 |
%|   L1 to/from L2 data volume [GBytes]   |   242.7314 | 
%|   L3 to L2 load bandwidth [MBytes/s]   |  3697.9893 | 
%|   L3 to L2 load data volume [GBytes]   |   181.1290 |  
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1201.2808 | 
%|   L2 to L3 evict data volume [GBytes]  |    58.8392 | 
%|   L2 to/from L3 bandwidth [MBytes/s]   |  4899.2701 | 
%|   L2 to/from L3 data volume [GBytes]   |   239.9682 |
%
%3T
%ADD_nOL
%+----------------------------------------+------------+-----------+
%|           Runtime (RDTSC) [s]          |    47.8892 |   48.0013 |
%|          Runtime unhalted [s]          |    47.1408 |   47.2976 |
%|               Clock [MHz]              |  2199.7990 | 2199.8906 |
%|                   CPI                  |     5.0158 |    5.1917 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  5067.6816 | 5055.9241 |
%|   L2 to L1 load data volume [GBytes]   |   242.6872 |  242.6909 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1688.4151 | 1683.4988 |
%|   L1 to L2 evict data volume [GBytes]  |    80.8568 |   80.8101 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  6756.0967 | 6739.4229 |
%|   L1 to/from L2 data volume [GBytes]   |   323.5440 |  323.5010 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  5019.5746 | 5010.1334 |
%|   L3 to L2 load data volume [GBytes]   |   240.3834 |  240.4929 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1634.6991 | 1631.7348 |
%|   L2 to L3 evict data volume [GBytes]  |    78.2844 |   78.3254 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  6654.2737 | 6641.8682 |
%|   L2 to/from L3 data volume [GBytes]   |   318.6678 |  318.8182 |
%WAXBPY_nOL
%+----------------------------------------+------------+-----------+
%|           Runtime (RDTSC) [s]          |    47.5941 |   47.4597 |
%|          Runtime unhalted [s]          |    47.0425 |   46.9324 |
%|               Clock [MHz]              |  2199.7990 | 2199.8906 |
%|                   CPI                  |     3.6291 |    3.6777 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  5099.3631 | 5113.7100 |
%|   L2 to L1 load data volume [GBytes]   |   242.6996 |  242.6950 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1698.6102 | 1702.4411 |
%|   L1 to L2 evict data volume [GBytes]  |    80.8438 |   80.7973 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  6797.9733 | 6816.1511 |
%|   L1 to/from L2 data volume [GBytes]   |   323.5435 |  323.4924 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  5046.0859 | 5062.5150 |
%|   L3 to L2 load data volume [GBytes]   |   240.1640 |  240.2653 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1638.7399 | 1646.1205 |
%|   L2 to L3 evict data volume [GBytes]  |    77.9944 |   78.1244 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  6684.8258 | 6708.6355 |
%|   L2 to/from L3 data volume [GBytes]   |   318.1583 |  318.3897 |
%ADD_OLWAXPBY
%|           Runtime (RDTSC) [s]          |   47.5143 |
%|          Runtime unhalted [s]          |   46.8081 |
%|               Clock [MHz]              | 2199.9154 |
%|                   CPI                  |    5.1239 |
%|   L2 to L1 load bandwidth [MBytes/s]   | 5107.7041 |
%|   L2 to L1 load data volume [GBytes]   |  242.6888 |
%|   L1 to L2 evict bandwidth [MBytes/s]  | 1701.6126 |
%|   L1 to L2 evict data volume [GBytes]  |   80.8509 |
%|   L1 to/from L2 bandwidth [MBytes/s]   | 6809.3167 |
%|   L1 to/from L2 data volume [GBytes]   |  323.5397 |
%|   L3 to L2 load bandwidth [MBytes/s]   | 5059.6404 |
%|   L3 to L2 load data volume [GBytes]   |  240.4051 |
%|   L2 to L3 evict bandwidth [MBytes/s]  | 1646.3561 |
%|   L2 to L3 evict data volume [GBytes]  |   78.2254 |
%|   L2 to/from L3 bandwidth [MBytes/s]   | 6705.9965 |
%|   L2 to/from L3 data volume [GBytes]   |  318.6305 |
%WAXPBY_OLADD 6.4 % decrease
%+----------------------------------------+------------+
%|           Runtime (RDTSC) [s]          |    50.8553 | 
%|          Runtime unhalted [s]          |    49.9441 | 
%|               Clock [MHz]              |  2199.6562 | 
%|                   CPI                  |     3.5741 |  
%|   L2 to L1 load bandwidth [MBytes/s]   |  4773.1203 |
%|   L2 to L1 load data volume [GBytes]   |   242.7384 | 
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1589.0072 |
%|   L1 to L2 evict data volume [GBytes]  |    80.8094 | 
%|   L1 to/from L2 bandwidth [MBytes/s]   |  6362.1275 |
%|   L1 to/from L2 data volume [GBytes]   |   323.5478 | 
%|   L3 to L2 load bandwidth [MBytes/s]   |  4722.0288 | 
%|   L3 to L2 load data volume [GBytes]   |   240.1401 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1532.3533 | 
%|   L2 to L3 evict data volume [GBytes]  |    77.9283 | 
%|   L2 to/from L3 bandwidth [MBytes/s]   |  6254.3821 | 
%|   L2 to/from L3 data volume [GBytes]   |   318.0684 
%
%2T
%ADD_nOL
%+----------------------------------------+------------+-----------+
%|           Runtime (RDTSC) [s]          |    51.4819 |   51.5248 |
%|          Runtime unhalted [s]          |    50.8195 |   50.8986 |
%|               Clock [MHz]              |  2199.9768 | 2199.7639 |
%|                   CPI                  |     3.6627 |    3.7458 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  7068.9996 | 7063.0176 |
%|   L2 to L1 load data volume [GBytes]   |   363.9252 |  363.9206 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  2354.5406 | 2353.3008 |
%|   L1 to L2 evict data volume [GBytes]  |   121.2161 |  121.2534 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  9423.5402 | 9416.3184 |
%|   L1 to/from L2 data volume [GBytes]   |   485.1414 |  485.1740 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  6923.4210 | 6928.6562 |
%|   L3 to L2 load data volume [GBytes]   |   356.4306 |  356.9977 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  2256.4133 | 2257.7445 |
%|   L2 to L3 evict data volume [GBytes]  |   116.1644 |  116.3299 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  9179.8343 | 9186.4007 |
%|   L2 to/from L3 data volume [GBytes]   |   472.5949 |  473.3276 |
%WAXBPY_nOL
%+----------------------------------------+------------+-----------+
%|           Runtime (RDTSC) [s]          |    51.0858 |   51.1941 |
%|          Runtime unhalted [s]          |    50.4809 |   50.5927 |
%|               Clock [MHz]              |  2199.9787 | 2199.7639 |
%|                   CPI                  |     2.6565 |    2.6685 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  7124.9649 | 7109.9393 |
%|   L2 to L1 load data volume [GBytes]   |   363.9843 |  363.9869 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  2372.5846 | 2367.4328 |
%|   L1 to L2 evict data volume [GBytes]  |   121.2053 |  121.1986 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  9497.5496 | 9477.3721 |
%|   L1 to/from L2 data volume [GBytes]   |   485.1896 |  485.1855 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  6972.9596 | 6962.4936 |
%|   L3 to L2 load data volume [GBytes]   |   356.2190 |  356.4386 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  2270.8389 | 2267.9964 |
%|   L2 to L3 evict data volume [GBytes]  |   116.0076 |  116.1080 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  9243.7984 | 9230.4899 |
%|   L2 to/from L3 data volume [GBytes]   |   472.2266 |  472.5466 |
%ADD_OLWAXPBY (No change)
%+----------------------------------------+-----------+
%|           Runtime (RDTSC) [s]          |   51.5216 |
%|          Runtime unhalted [s]          |   50.9150 |
%|               Clock [MHz]              | 2199.9819 |
%|                   CPI                  |    3.7822 |
%|   L2 to L1 load bandwidth [MBytes/s]   | 7063.6887 |
%|   L2 to L1 load data volume [GBytes]   |  363.9325 |
%|   L1 to L2 evict bandwidth [MBytes/s]  | 2352.6251 |
%|   L1 to L2 evict data volume [GBytes]  |  121.2110 |
%|   L1 to/from L2 bandwidth [MBytes/s]   | 9416.3138 |
%|   L1 to/from L2 data volume [GBytes]   |  485.1436 |
%|   L3 to L2 load bandwidth [MBytes/s]   | 6924.0694 |
%|   L3 to L2 load data volume [GBytes]   |  356.7391 |
%|   L2 to L3 evict bandwidth [MBytes/s]  | 2256.7324 |
%|   L2 to L3 evict data volume [GBytes]  |  116.2705 |
%|   L2 to/from L3 bandwidth [MBytes/s]   | 9180.8018 |
%|   L2 to/from L3 data volume [GBytes]   |  473.0096 |
%WAXPBY_OLADD 2.3 % decrease
%|           Runtime (RDTSC) [s]          |    52.3063 | 
%|          Runtime unhalted [s]          |    51.4637 |  
%|               Clock [MHz]              |  2199.8976 |
%|                   CPI                  |     2.6574 | 
%|   L2 to L1 load bandwidth [MBytes/s]   |  6959.1242 | 
%|   L2 to L1 load data volume [GBytes]   |   364.0058 | 
%|   L1 to L2 evict bandwidth [MBytes/s]  |  2317.2838 | 
%|   L1 to L2 evict data volume [GBytes]  |   121.2084 | 
%|   L1 to/from L2 bandwidth [MBytes/s]   |  9276.4080 |
%|   L1 to/from L2 data volume [GBytes]   |   485.2142 | 
%|   L3 to L2 load bandwidth [MBytes/s]   |  6807.2960 | 
%|   L3 to L2 load data volume [GBytes]   |   356.0642 |  
%|   L2 to L3 evict bandwidth [MBytes/s]  |  2213.9355 | 
%|   L2 to L3 evict data volume [GBytes]  |   115.8027 |  
%|   L2 to/from L3 bandwidth [MBytes/s]   |  9021.2315 | 
%|   L2 to/from L3 data volume [GBytes]   |   471.8669
%
%1T
%ADD_nOL
%+----------------------------------------+------------+------------+
%|           Runtime (RDTSC) [s]          |    80.6170 |    81.1784 |
%|          Runtime unhalted [s]          |    80.0828 |    80.6588 |
%|               Clock [MHz]              |  2199.9767 |  2199.8158 |
%|                   CPI                  |     3.0010 |     3.0224 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  9026.2535 |  8963.2614 |
%|   L2 to L1 load data volume [GBytes]   |   727.6691 |   727.6230 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  3006.7162 |  2986.7271 |
%|   L1 to L2 evict data volume [GBytes]  |   242.3923 |   242.4577 |
%|   L1 to/from L2 bandwidth [MBytes/s]   | 12032.9697 | 11949.9885 |
%|   L1 to/from L2 data volume [GBytes]   |   970.0614 |   970.0807 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  8781.8901 |  8739.9349 |
%|   L3 to L2 load data volume [GBytes]   |   707.9693 |   709.4938 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  2875.5692 |  2862.5324 |
%|   L2 to L3 evict data volume [GBytes]  |   231.8196 |   232.3757 |
%|   L2 to/from L3 bandwidth [MBytes/s]   | 11657.4593 | 11602.4674 |
%|   L2 to/from L3 data volume [GBytes]   |   939.7889 |   941.8695 |
%WAXBPY_nOL
%+----------------------------------------+------------+------------+
%|           Runtime (RDTSC) [s]          |    81.8850 |    82.1917 |
%|          Runtime unhalted [s]          |    80.5689 |    80.8980 |
%|               Clock [MHz]              |  2199.9742 |  2199.8145 |
%|                   CPI                  |     2.1767 |     2.1854 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  8892.3984 |  8860.1619 |
%|   L2 to L1 load data volume [GBytes]   |   728.1536 |   728.2317 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  2959.7015 |  2949.4719 |
%|   L1 to L2 evict data volume [GBytes]  |   242.3550 |   242.4221 |
%|   L1 to/from L2 bandwidth [MBytes/s]   | 11852.0999 | 11809.6338 |
%|   L1 to/from L2 data volume [GBytes]   |   970.5086 |   970.6538 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  8639.2510 |  8622.1466 |
%|   L3 to L2 load data volume [GBytes]   |   707.4246 |   708.6688 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  2825.5972 |  2819.9569 |
%|   L2 to L3 evict data volume [GBytes]  |   231.3739 |   231.7770 |
%|   L2 to/from L3 bandwidth [MBytes/s]   | 11464.8483 | 11442.1035 |
%|   L2 to/from L3 data volume [GBytes]   |   938.7985 |   940.4458 |
%ADD_OLWAXPBY (No change)
%+----------------------------------------+------------+
%|           Runtime (RDTSC) [s]          |    81.4527 |
%|          Runtime unhalted [s]          |    80.9078 |
%|               Clock [MHz]              |  2199.9798 |
%|                   CPI                  |     3.0320 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  8932.9770 |
%|   L2 to L1 load data volume [GBytes]   |   727.6154 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  2976.7347 |
%|   L1 to L2 evict data volume [GBytes]  |   242.4632 |
%|   L1 to/from L2 bandwidth [MBytes/s]   | 11909.7117 |
%|   L1 to/from L2 data volume [GBytes]   |   970.0785 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  8710.6541 |
%|   L3 to L2 load data volume [GBytes]   |   709.5066 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  2852.9733 |
%|   L2 to L3 evict data volume [GBytes]  |   232.3825 |
%|   L2 to/from L3 bandwidth [MBytes/s]   | 11563.6274 |
%|   L2 to/from L3 data volume [GBytes]   |   941.8890 |
%WAXPBY_OLADD (No change)
%|           Runtime (RDTSC) [s]          |    81.8278 |
%|          Runtime unhalted [s]          |    80.8142 |
%|               Clock [MHz]              |  2199.9394 |
%|                   CPI                  |     2.1832 |  
%|   L2 to L1 load bandwidth [MBytes/s]   |  8898.0124 |  
%|   L2 to L1 load data volume [GBytes]   |   728.1050 | 
%|   L1 to L2 evict bandwidth [MBytes/s]  |  2963.1178 |
%|   L1 to L2 evict data volume [GBytes]  |   242.4655 | 
%|   L1 to/from L2 bandwidth [MBytes/s]   | 11861.1303 |
%|   L1 to/from L2 data volume [GBytes]   |   970.5704 | 
%|   L3 to L2 load bandwidth [MBytes/s]   |  8648.7006 | 
%|   L3 to L2 load data volume [GBytes]   |   707.7043 |  
%|   L2 to L3 evict bandwidth [MBytes/s]  |  2827.8375 | 
%|   L2 to L3 evict data volume [GBytes]  |   231.3958 | 
%|   L2 to/from L3 bandwidth [MBytes/s]   | 11476.5381 | 
%|   L2 to/from L3 data volume [GBytes]   |   939.1001 |
 

==> tables/tab1_overlap.tex <==
\setlength\tabcolsep{0.5pt}
\setlength\extrarowheight{-0.2pt}
\arrayrulecolor{Blue}
\begin{tabular}[fragile]{|l|c|c|c|c|c|}
	\toprule	
	\rowcolor[gray]{0.9}
	{Regime} & {Kernels} &\multicolumn{3}{c|}{Memory pressure $P_\mathrm{MEM}$}& {Overlapping}  \\
	\rowcolor[gray]{0.9}
	& {Applicability} & \multicolumn{3}{c|}{$P_\mathrm{MEM}=T_\mathrm{L3-MEM}\mbox{$\mathparagraph$} / T$} & Performance \\
	\midrule
	\cellcolor{Cyan!10!white} 
							& A & \multicolumn{3}{c|}{$\leq$ 50 \%} & {No change}  \\
	\multirow{-2}{*}{\cellcolor{Cyan!10!white}Scalable}
							& B & \multicolumn{3}{c|}{$\leq$ 50 \%} & No change  \\ \cline{1-6}
 
							& A & \multicolumn{3}{c|}{$\leq$ 50 \%} & No change \\ 
							\cellcolor{Cyan!10!white}& B & \multicolumn{3}{c|}{$>$ 50 \%\mbox{$\dagger$}} & Speedup \\ \cline{2-6}
							\multirow{-2}{*}{\cellcolor{Cyan!10!white}Bottleneck}& A &  $>$ 50 \% &  $>$ 50 & $=$ 100 \% & Speedup(/slowdown) \\ 
							& B & $>$ 50 \% & $=$ 100 \%\mbox{$\S$}  & $=$ 100 \% & Slowdown(/speedup) \\ 
	\bottomrule
\end{tabular}

==> tables/tab2_cases.tex <==
\setlength\extrarowheight{-100pt}
\begin{tabular}[fragile]{|l|c|c|c|}
	\toprule
	\rowcolor[gray]{0.9}
	{Cases} & {Kernels} & {Memory pressure $P_\mathrm{MEM}$\mbox{$\S$}} & {Saturated bandwidth $B_s$} \\
	\midrule
	\cellcolor{Cyan!10!white} 
							& A & High & Same  \\ %\cline{2-4}
	\multirow{-5}{*}{\cellcolor{Cyan!10!white}First}						
							& B & Low & Same  \\ 
	\midrule
	\cellcolor{Cyan!10!white}
						 	& A & High & High \\ %\cline{2-4}
	\multirow{-5}{*}{\cellcolor{Cyan!10!white}Second}						
							& B & Low & Low \\ 
	\midrule
	\cellcolor{Cyan!10!white} 
							& A & High & Low \\ %\cline{2-4}
	\multirow{-5}{*}{\cellcolor{Cyan!10!white}Third}						
							& B & Low & High \\ 
	\bottomrule
\end{tabular}

==> tables/tab4_ECM.tex <==
\setlength\tabcolsep{0.5pt}
\setlength\extrarowheight{0pt} 
\arrayrulecolor{Blue}

\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}clc}
%\begin{tabular}[fragile]{|l|l|c|c|c|c|}
	\specialrule{2.5pt}{1pt}{1pt}
	 \rowcolor[gray]{0.85}
	 &  & {Multi-core ECM model\mbox{$\S$}}  	\\
	 \rowcolor[gray]{0.9}
	&&   Perf $=$ $\frac{n \times iter \times \si{f} \times \si{\flop} }{C1\mbox{$\dagger$}|C2|C3|C4|C5|C6|C7|C8|C9|C10}$ { [\si{\flop\per\second}]} \\ 
	\rowcolor[gray]{0.9}
	&{Kernels} &  $b_\mathrm{MEM}$ $=$  ${b1|b2|b3|b4|b5|b6|b7|b8|b9|b10}$ {[\si{\giga \bytes\per\second}]}  \\
	\rowcolor[gray]{0.9}
	&&  $P_\mathrm{MEM}$ $=$  ${P1|P2|P3|P4|P5|P6|P7|P8|P9|P10}$ {[\%]}  \\
	\specialrule{2.5pt}{1pt}{1pt}
	&\cellcolor{Cyan!10!white} DDOT
							 & \normalsize{$(4.4 \times iter) / (\max(3, (4 + 4 + 4 + 6))|9.5|7.3|6.4|\textbf{6}|6|6|6|6|6)$} \\ 
							 \cellcolor[gray]{0.9}&& \normalsize{$15.6$
							\mbox{$\ddagger$}
							$|29.64|38.57|44|\textbf{46.9}$
							\mbox{$\mathparagraph$}
							$|46.9 |46.9 |46.9 |46.9 |46.9 $}  \\
							\cellcolor[gray]{0.9}&&\normalsize{$33.26|63.2|82.2|93.8|\textbf{100}|100|100|100|100|100$}\\
							 \cline{2-3}
	\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white} vectorSUM  
							 & \normalsize{$(2.2 \times iter) / (\max(2, (2 + 2 + 2 + 3))|4.7   | 3.6   | 3.2   | \textbf{3}   | 3   | 3   | 3   | 3   | 3)$} \\ 
							 \cellcolor[gray]{0.9}&& 
							 \normalsize{$15.64 | 29.957| 39.1| 44| \textbf{46.9}| 46.9| 46.9 | 46.9 |46.9 |46.9$} \\ 
 							\multirow{-6}{*}{\rotatebox{90}{Read-only}}&&\normalsize{$33.3|63.87|83.37|93.8|\textbf{100}|100|100|100|100|100$}\\
 
	\specialrule{1.65pt}{0.15pt}{0.15pt}
	&\cellcolor{Cyan!10!white} {DSCAL}    
							 & \normalsize{$(2.2 \times iter) / (\max(4, (2 + 4 + 4 + 7.5))|9.6  | 7.8  | \textbf{7.5}  | 7.5  | 7.5  | 7.5  | 7.5  | 7.5  | 7.5) 
							 	$} \\
						 	&&  \normalsize{$16.09 | 29.33| 36.1| \textbf{37.54}| 37.54| 37.54| 37.54 | 37.54 |37.54 |37.54$} \\ 
							 &&\normalsize{$42.86|78.13|96.16|\textbf{100}|100|100|100|100|100|100$}\\
							  \cline{2-3}
	&\cellcolor{Cyan!10!white} {DAXPY}   
							 & \normalsize{$(4.4 \times iter) / (\max(4.2, (4 + 6 + 6 + 10.3))|14.1  | 11.2  | \textbf{10.3}  | 10.3  | 10.3  | 10.3  | 10.3  | 10.3  | 10.3) 
							$} \\
							 &&  \normalsize{$16.06 | 29.96| 37.7| \textbf{41}| 41| 41| 41 | 41 |41 |41$} \\
							 &&\normalsize{$39.17|73.07|91.95|\textbf{100}|100|100|100|100|100|100$}\\
							  \cline{2-3}
	&\cellcolor{Cyan!10!white} {ADD}    
							  & \normalsize{$(2.2 \times iter) / (\max(5, (4 + 8 + 8 + 13.7))|18.2  | 14.7  | \textbf{13.7}  | 13.7  | 13.7  | 13.7  | 13.7  | 13.7  | 13.7 )$}  \\ 
							 &&  \normalsize{$16.7 | 30.9| 38.3| \textbf{41.1}| 41.1| 41.1| 41.1 | 41.1 |41.1 |41.1$} \\
							 &&\normalsize{$40.6|75.18|93.2|\textbf{100}|100|100|100|100|100|100$}\\
							   \cline{2-3}
	&\cellcolor{Cyan!10!white} {STREAM}    
							  & \normalsize{$(4.4 \times iter) / (\max(5.2, (4 + 8 + 8 + 13.7))|18.2|14.7|\textbf{13.7}|13.7|13.7|13.7|13.7|13.7)$}  \\ 
							 &&  \normalsize{$16.7|30.9|38.3|\textbf{41.1}|41.1|41.1|41.1|41.1|41.1|41.1$} \\
							  &&  \normalsize{$40.7 |75.3 |93.2|\textbf{100}|100|100|100|100|100|100$}
							\\ \cline{2-3}
	&\cellcolor{Cyan!10!white} {WAXPBY}    
							 & \normalsize{$(6.6 \times iter) / (\max(5.2, (4 + 8 + 8 + 13.7))|18.2|14.7|\textbf{13.7}|13.7|13.7|13.7|13.7|13.7)$} \\ 
							 && \normalsize{$16.7|30.9|38.3|\textbf{41.1}|41.1|41.1|41.1|41.1|41.1|41.1$}\\  
							 \cellcolor[gray]{0.9}&&\normalsize{$40.63|75.18|93.2|\textbf{100}|100|100|100|100|100|100$}\\
							 \cline{2-3}
	\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white} {DCOPY}   
							 &  \normalsize{$\max(5, (2 + 6 + 6 + 10.3))|13.2  | 10.7  | \textbf{10.3}  | 10.3  | 10.3  | 10.3  | 10.3  | 10.3  | 10.3 $} [\si{\cycles}]\\ 
							 \cellcolor[gray]{0.9}&&  \normalsize{$17.4 | 32| 39.48| \textbf{41}| 41| 41| 41 | 41 |41 |41$} \\
							 \cellcolor[gray]{0.9}&&\normalsize{$42.43|78|96.29|\textbf{100}|100|100|100|100|100|100$}\\
							 \cline{2-3}
	\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white} {Schoenauer}    
							  &  \normalsize{$(4.4 \times iter) / (\max(7, (6 + 10 + 10 + 16.8))|23.1  | 18.4  | \textbf{16.8}  | 16.8  | 16.8  | 16.8  | 16.8  | 16.8  | 16.8) $}\\ 
							 &&  \normalsize{$16.45 | 30.47| 38.26| \textbf{41.9}| 41.9| 41.9| 41.9 | 41.9 |41.9 |41.9$} \\
							 &&\normalsize{$39.26|72.7|91.3|\textbf{100}|100|100|100|100|100|100$}\\
							 \cline{2-3}
	&\cellcolor{Cyan!10!white} {Jacobi-v1}   
							& \normalsize{$(8.8 \times iter \times D_\mathrm{inner} \times D_\mathrm{outer})/(\max(9.4, (8+10+6+10.3))|17.9  | 13.4  | 11.5  | 10.5  | \textbf{10.3}  | 10.3  | 10.3  | 10.3  | 10.3)$}  \\ 
							&\multirow{2}{*}{$LC_\mathrm{L2}$ $\checkmark$}&  \normalsize{$12.3| 23.6 |31.52 | 36.73| 40.22| \textbf{41}| 41|  41 |41 |41$} \\
							&& \normalsize{$30|57.56|76.88|89.58|98.1|\textbf{100}|100|100|100|100$}\\ \cline{2-3}
	&\cellcolor{Cyan!10!white} {Jacobi-v2}   
							& \normalsize{$(8.8 \times iter \times D_\mathrm{inner} \times D_\mathrm{outer})/(\max(56, (12+12+8+13.7))|28.8  | 20.8  | 17.4  | 15.5  | 14.4  | \textbf{13.7}  | 13.7  | 13.7  | 13.7)$}  \\ 
							&\multirow{2}{*}{$LC_\mathrm{L2}$ $\checkmark$}&  \normalsize{$8.99 | 19.55| 27.08 | 32.37| 36.34| 39.1| \textbf{41.1}| 41.1 |41.1 |41.1$} \\
							&& \normalsize{$21.87|47.57|65.89|78.76|88.42|95.13|\textbf{100}|100|100|100$}\\ 
							 \cline{2-3}
	&\cellcolor{Cyan!10!white} {Jacobi-v1}   
							& \normalsize{$(8.8 \times iter \times D_\mathrm{inner} \times D_\mathrm{outer})/(\max(9.4, (8+ 10+10+10.3))|19.8|14.5|12.3|11.1|\textbf{10.3}|10.3|10.3|10.3|10.3)$}  \\ 
							&\multirow{2}{*}{$LC_\mathrm{L3}$ $\checkmark$}&  \normalsize{$11 | 21.3| 29.1| 34.3| 38.05| \textbf{41.1}| 41.1 | 41.1 |41.1 |41.1$} \\
							&& \normalsize{$26.9|52|71|83.7|92.8|\textbf{100}|100|100|100|100$}\\ \cline{2-3}
	&\cellcolor{Cyan!10!white} {Jacobi-v2}   
							& \normalsize{$(28.6 \times iter \times D_\mathrm{inner} \times D_\mathrm{outer})/(\max(56, (12+12+12+13.4))| 28.8  | 20.8  | 17.3  | 15.4  | 14.2  | \textbf{13.4}  | 13.4  | 13.4  | 13.4 )$}  \\ 
							&\multirow{2}{*}{$LC_\mathrm{L3}$ $\checkmark$}&  \normalsize{$11.4 | 19.55 |27.08 | 32.55 | 36.57| 39.66| \textbf{42.03}| 42.03 | 42.03 |42.03$}\\ 
							\multirow{-33}{*}{\rotatebox{90}{Read-write}}&& \normalsize{$27.12|46.51|64.43|77.44|87|94.36|\textbf{100}|100|100|100$}\\
	\specialrule{2.5pt}{1pt}{1pt}
%\end{tabular}
\end{tabular*}


==> tables/tab5_OBM.tex <==
\setlength\tabcolsep{0pt}
\setlength\extrarowheight{0pt} 
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}|c|c|cccccc|cc|cc|}
	\specialrule{2.5pt}{1pt}{1pt}
	\rowcolor[gray]{0.9}
	& &{Overlapping cases\mbox{$\ast$}}  & $\delta P^\mathrm{CA-C1}_\mathrm{MEM}$ 
	& $\delta b^\mathrm{CA}_s$ 
	& $\delta b^\mathrm{CB}_s$ 
	& $\delta R+\delta W+\delta WA$ & $\delta B_{c}$ 
	& \multicolumn{4}{c}{Average bandwidth change\mbox{$\S$}} \\
	\rowcolor[gray]{0.9}
	&
	& {KerA+KerB\mbox{$\mathparagraph$}}  
	& [\%] 
	& [$\frac{\GB}{s}$] 
	& [$\frac{\GB}{s}$]  
	& [$\frac{B}{row}$] 
	&  
	& {$\bar b^\mathrm{CA}_\mathrm{KerA}$ [\%]}   
	& {$\bar b^\mathrm{CA}_\mathrm{KerB}$ [\%]} 
	& {$\bar b^\mathrm{CB}_\mathrm{KerA}$ [\%]}  
	& {$\bar b^\mathrm{CB}_\mathrm{KerB}$ [\%]} \\
	\specialrule{2.5pt}{1pt}{1pt}
	
	& 
	&\cellcolor{Cyan!10!white}STREAM+Jacobi-v2($LC_\mathrm{L3}$ $\checkmark$)  & 	-16.8
%	 \hspace{0.85cm}	-16.8
%	\multirow{1}{*}{\begin{tikzpicture}[baseline=(current bounding box.east)]
%		\draw [thick, red,decorate,decoration={brace,amplitude=10pt,mirror},rotate=90,xshift=-20pt,yshift=12pt](0,0) -- (2.5,0) node[black,midway,rotate=90,yshift=-0.6cm] {\footnotesize $\pmb{\delta P_\mathrm{MEM}}$};	
%		\end{tikzpicture}}
	& 0.93  & & 
	-- &  $\div$6.5 & 1.46$\uparrow$ & -- &&\\ \cline{9-10}\cline{11-12}

%	STREAM\_nOL (300M vector size): 
%	47.8889 |   47.8927 s, 47.5495 |   47.4770 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4053.4865 | 4053.9498 MB/s,  4082.4254 | 4089.1390 
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4009.9707 | 4007.8148 MB/s,  4039.2496 | 4044.2358
%	$b_\mathrm{MEM}=40677(30502+10174) MB/s.
%	STREAM\_OL (300M vector size): 1.46 % increse
%	47.7145 s, 47.2039 
%	$b_\mathrm{L1 \rightleftarrows L2}$=  4069.2362 MB/s, 4112.9724 
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4022.5963 MB/s. 4066.6949
%	Jacobi\_nOL (300M vector size): 
%	55.9920 |   56.0862 s,  55.8071 |   55.9468
%	$b_\mathrm{L1 \rightleftarrows L2}$= 6208.8867 | 6199.4020 MB/s, 6229.5725 | 6214.9999
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4093.3772 | 4086.2111 MB/s,  4108.9783 | 4096.4502 
%	$b_\mathrm{MEM}=41352(31012+10340) MB/s.
%	Jacobi\_OL (300M vector size): No change
%	56.4822 s,  56.1339
%	$b_\mathrm{L1 \rightleftarrows L2}$= 6152.8109 MB/s, 6193.3673 
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4052.8269 MB/s, 4083.5135
%	$b_\mathrm{MEM}=41028(30766+10261) MB/s.

	&&\cellcolor{Cyan!10!white}STREAM+Jacobi-v2($LC_\mathrm{L2}$ $\checkmark$) & -16.2&  -- & &
	--
	&  
	\hspace{1cm}$\div$6.5
	\multirow{1}{*}{\begin{tikzpicture}[baseline=(current bounding box.east)]
		\draw [thick, red,decorate,decoration={brace,amplitude=10pt,mirror},rotate=90,xshift=-20pt,yshift=12pt](0,0) -- (0.75,0) node[black,midway,rotate=90,yshift=-0.6cm] {\footnotesize $\pmb{\delta B_c}$};	
		\end{tikzpicture}}
	& 5$\uparrow$ &6$\downarrow$ &&  \\ \cline{9-10}\cline{11-12}

%	STREAM\_nOL (300M vector size): 
%	47.7255 |   47.7835 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4068.1264 | 4062.3463 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4022.4293 | 4018.9242 MB/s,
%	$b_\mathrm{MEM}=40790(30587+10203) MB/s.
%	STREAM\_OL (300M vector size): 
%	45.3043  s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$=4284.7464 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$=4232.6777 MB/s.
%	Jacobi\_nOL (300M vector size): 
%	56.4562 |   56.9638 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 6156.0253 | 6101.8255  MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 6108.2719 | 6056.6971 MB/s,
%	$b_\mathrm{MEM}=41187(30976+10211) MB/s.
%	Jacobi\_OL (300M vector size): 
%	59.9241 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$=5799.0799  MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$=5753.9419  MB/s,
%	$b_\mathrm{MEM}=41035(30789+10245) MB/s.	

	&\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white}STREAM+Jacobi-v1($LC_\mathrm{L3}$ $\checkmark$)  & -13.8 & -- & &
		\hspace{0.65cm} -1+0+0
	\multirow{1}{*}{\begin{tikzpicture}[baseline=(current bounding box.east)]
		\draw [thick, red,decorate,decoration={brace,amplitude=10pt,mirror},rotate=90,xshift=-20pt,yshift=12pt](0,0) -- (1.7,0) node[black,midway,rotate=90,yshift=-0.6cm] {\footnotesize $\pmb{\delta R}$};	
		\end{tikzpicture}}
	& $\div$2.67 &2.7$\downarrow$  & 3.3$\uparrow$ && \\ \cline{9-10}\cline{11-12}

%	STREAM\_nOL (300M vector size): 
%	 47.8206 |   47.8537  s, 47.3373 |   47.3005
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4059.5292 | 4057.3586  MB/s, 4101.5245 | 4103.9175
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4015.2346 | 4011.3185 MB/s, 4054.4414 | 4060.1288
%	$b_\mathrm{MEM}=40720(30534+10185) MB/s.
%	STREAM\_OL (300M vector size): 
%	48.8823 s, 48.6588
%	$b_\mathrm{L1 \rightleftarrows L2}$= 3972.0269 MB/s, 3990.1086
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3925.6797 MB/s.  3943.2745
%	Jacobi\_nOL (300M vector size): 
%	 43.4633 |   43.3744 s, 43.0638 |   43.1187
%	$b_\mathrm{L1 \rightleftarrows L2}$= 6646.5778 | 6661.4406 MB/s, 6708.8031 | 6700.0237
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3898.4973 | 3907.7256 MB/s, 3931.3831 | 3933.5215
%	$b_\mathrm{MEM}=40006(26686+13319) MB/s.
%	Jacobi\_OL (300M vector size): 
%	 41.8895 s,  41.7055
%	$b_\mathrm{L1 \rightleftarrows L2}$= 6895.9537 MB/s, 6927.3653
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4047.8615 MB/s, 4063.8538
%	$b_\mathrm{MEM}=40599(28725+11873) MB/s.

	&\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white}STREAM+Jacobi-v1($LC_\mathrm{L2}$ $\checkmark$) & -10.7 & -0.1& & -1+0+0 &  
	\hspace{0.85cm}$\div$2.67
	\multirow{1}{*}{\begin{tikzpicture}[baseline=(current bounding box.east)]
		\draw [thick, red,decorate,decoration={brace,amplitude=10pt,mirror},rotate=90,xshift=-20pt,yshift=12pt](0,0) -- (1,0) node[black,midway,rotate=90,yshift=-0.6cm] {\footnotesize $\pmb{\delta B_c}$};	
		\end{tikzpicture}}
	&  4.5$\uparrow$ &4.5$\downarrow$ && \\ \cline{9-10}\cline{11-12}
%	STREAM\_nOL (300M vector size): 
%	 47.5722 |   47.6834 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4080.5668 | 4071.7913 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4036.1823 | 4025.0381 MB/s,
%	$b_\mathrm{MEM}=40896(30666+10229) MB/s.
%	STREAM\_OL (300M vector size): 
%	45.4290 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4273.7577 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4213.5954 MB/s.
%	Jacobi\_nOL (300M vector size): 
%	43.1944 |   43.1603 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 6679.8376 | 6688.9514  MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 6613.5833 | 6625.9596 MB/s,
%	$b_\mathrm{MEM}=40635(27230+13404) MB/s.
%	Jacobi\_OL (300M vector size): 
%	 45.2956  s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 6370.0563 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 6317.0620 MB/s,
%	$b_\mathrm{MEM}=40769(28995+11773) MB/s.

	&\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white}DSCAL+DAXPBY & -3.6 & 3.46 & & 1+0+0  & $\div$1.33 &   8$\uparrow$ & $7.5\downarrow$&  12.5$\uparrow$& $9\downarrow$ \\
	\cline{9-10}\cline{11-12}
%	DSCAL\_nOL (300M vector size): 
%	26.3295 |   26.3335 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 3676.2048 | 3675.3304 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3549.7991 | 3549.9488  MB/s,
%	$b_\mathrm{MEM}=36958(18508+18450) MB/s.
%	DSCAL\_OL (300M vector size): 
%	24.3965 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 3971.8277  MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3879.3062 MB/s.
%	DAXPBY\_nOL (300M vector size): 
%	 36.1283 |   36.1343s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4034.6472 | 4034.0254 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3982.3862 | 3981.8556 MB/s,
%	$b_\mathrm{MEM}=40445(26973+13471) MB/s.
%	DAXPBY\_OL (300M vector size): 
%	 39.0450  s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 3733.0574 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3680.4517 MB/s,
%	$b_\mathrm{MEM}=(+) MB/s.

	&\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white}STREAM+Schoenauer & -1.45 & 0.8 & & 1+0+0  & $\times$1.33 &6.5$\uparrow$ &10.5$\downarrow$ &6.1$\uparrow$ & 9.6$\downarrow$  \\ 
	\cline{4-7}
	\cline{8-11}
%	Schoenauer\_nOL (300M vector size): 
%	58.4099 |   58.3899 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4163.8064 | 4164.6428 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4124.3109 | 4126.6205 MB/s,
%	$b_\mathrm{MEM}=41680(33326+8354) MB/s.
%	Schoenauer\_OL (300M vector size): 
%	65.1944 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 3730.4426   MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3696.9321 MB/s.
%	$b_\mathrm{MEM}=40122(31002+9120) MB/s.
%	STREAM\_nOL (300M vector size): 
%	48.5600 |   48.6925 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4000.0084 | 3988.0782 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3956.1321 | 3947.5062 MB/s,
%	$b_\mathrm{MEM}=40120(30068+10052) MB/s.
%	STREAM\_OL (300M vector size): 
%	45.4922  s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4269.7493 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4221.9612 MB/s.


	&\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white}WAXBPY+ADD & 	\multirow{3}{*}{--}
	& \multirow{3}{*}{--} &  & \multirow{3}{*}{--}  & 
	\hspace{1cm}$\times$3
	\multirow{1}{*}{\begin{tikzpicture}[baseline=(current bounding box.east)]
		\draw [thick, red,decorate,decoration={brace,amplitude=10pt,mirror},rotate=90,xshift=-20pt,yshift=12pt](0,0) -- (1.15,0) node[black,midway,rotate=90,yshift=-0.6cm] {\footnotesize $\pmb{\delta B_c}$};	
		\end{tikzpicture}}
	& $\downarrow$ &  $\downarrow$ & -- & --\\ 
	\cline{9-10}
	\cline{11-12}

%	ADD\_nOL = STREAM\_OLWAXPBY = STREAM\_OLADD (300M vector size): 
%	50.1130 |   49.8105  s,  46.3863 |   48.2360
%	$b_\mathrm{L1 \rightleftarrows L2}$=   3876.0410 | 3898.1899 MB/s, 4189.4434 | 4026.9338
%	$b_\mathrm{L2 \rightleftarrows L3}$=   3831.4029 | 3854.9489 MB/s, 4147.0969 | 3982.1478
%	$b_\mathrm{MEM}=39273(29418+9854) MB/s. 40686.5652

%	ADD\_OLWAXPBY (300M vector size): 
%	53.5461  s, 48.2263 
%	$b_\mathrm{L1 \rightleftarrows L2}$=   3628.1360 MB/s, 4029.0193
%	$b_\mathrm{L2 \rightleftarrows L3}$=   3587.8240  MB/s, 3988.3768
%	$b_\mathrm{MEM}=40714.5973 MB/s.

%	WAXPBY\_nOL = WAXPBY\_OLSTREAM (300M vector size): 
%	47.6545 |   47.7963   s,  47.4428 |   47.7555 
%	$b_\mathrm{L1 \rightleftarrows L2}$=  4073.5530 | 4061.2090 MB/s,  4092.4407 | 4064.9475
%	$b_\mathrm{L2 \rightleftarrows L3}$=  4029.7303 | 4018.0930  MB/s,  4046.0930 | 4021.5968 
%	$b_\mathrm{MEM}=40738(30550+10187) MB/s.  40865.7068	

%	WAXPBY\_OLSTREAM (300M vector size): 
%	45.5966  47.5861 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4259.9989 MB/s, 4079.0975 
%	$b_\mathrm{L2 \rightleftarrows L3}$=  4206.7579 MB/s,4035.4069
%	$b_\mathrm{MEM}=39667(29712+9955) MB/s. 40812.7699

	&&\cellcolor{Cyan!10!white}WAXBPY+STREAM  & & --  &&  & $\times$1.5 &  5$\uparrow$  & 9.2$\downarrow$ & -- & -- \\  


	\cline{9-10}\cline{11-12}	
%	STREAM\_nOL = STREAM\_OLWAXPBY = STREAM\_OLADD (300M vector size): 
%	 46.3931 |   46.7145  s,  48.6439 |   46.0675
%	$b_\mathrm{L1 \rightleftarrows L2}$=   4191.1160 | 4161.9258 MB/s,  3995.9004 | 4220.1234
%	$b_\mathrm{L2 \rightleftarrows L3}$=   4147.5522 | 4119.6434 MB/s, 3938.1540 | 4173.6594
%	$b_\mathrm{MEM}= 40565.9713  MB/s. 38954.8972

%	STREAM\_OLWAXPBY (300M vector size): 
%	53.6185   s,  
%	$b_\mathrm{L1 \rightleftarrows L2}$=   3624.7075 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$=   3578.8566  MB/s,
%	$b_\mathrm{MEM}=39123.4403 MB/s.

%	WAXPBY\_nOL = WAXPBY\_OLSTREAM (300M vector size): 
%	47.6379 |   47.4471,  50.0096 |   47.7204 |
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4074.9125 | 4091.9998 MB/s, 3884.1865 | 4067.7585
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4030.9383 | 4045.1296 MB/s, 3838.9168 | 4023.7098 
%	$b_\mathrm{MEM}= 40797.2995 MB/s. 39168.2391 

%	WAXPBY\_OLSTREAM (300M vector size): 
%	45.3764  
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4280.6167 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4225.1343  MB/s,
%	$b_\mathrm{MEM}= 38849.3234 MB/s.

	&\multirow{-9}{*}{\rotatebox{90}{Read-write}}&\cellcolor{Cyan!10!white}STREAM+ADD & &  & &   & $\times$2 &3.5$\downarrow$ &  8.6$\downarrow$ & -- & -- \\ 
	\cmidrule[1.5pt]{2-11}
%	STREAM\_nOL (300M vector size): 
%	49.2285 |   49.2063, 47.5682 |   47.5845
%	$b_\mathrm{L1 \rightleftarrows L2}$=  3945.1771 | 3947.0797 MB/s, 4081.6038 | 4079.5309
%	$b_\mathrm{L2 \rightleftarrows L3}$=  3902.9666 | 3906.4332 MB/s, 4036.4327 | 4037.0020
%	$b_\mathrm{MEM}=39952(29962+9989) MB/s. 40811.6945
%	STREAM\_OLADD (300M vector size): 
%	  49.3232 
%	$b_\mathrm{L1 \rightleftarrows L2}$=  3937.5060  MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$=  3891.1991 MB/s.
%	$b_\mathrm{MEM}=38028.7784 MB/s.
%	ADD\_nOL = ADD\_OLSTREAM (300M vector size): 
%	48.3730 |   46.3108    s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$=  4014.6091 | 4195.6593   MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$=  3968.3563 | 4154.8880  MB/s,
%	$b_\mathrm{MEM}=40488.8594 MB/s.
%	ADD\_OLSTREAM (300M vector size): 
%	  52.9513  
%	$b_\mathrm{L1 \rightleftarrows L2}$= 3668.9650 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3632.3987 MB/s,
%	$b_\mathrm{MEM}=38781.1276 MB/s.

	& &\cellcolor{Cyan!10!white}DDOT1+VectorSUM & --
	& -- %1.6 Emmy 
	& --
	& 
  	--
	& $\times$2  & 3.5$\downarrow$ &  5$\downarrow$ & --  &  -- \\ 
	\cline{4-7}
	\cline{8-11}
%	DDOT1\_nOL (300M vector size): 
%	10.3590 |   10.3551  , 10.3538 |   10.3617
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4685.6500 | 4686.4134 MB/s, 4688.2793 | 4683.3688
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4610.5616 | 4611.3277 MB/s, 4612.3023 | 4608.0943
%	$b_\mathrm{MEM}=  47016.3675  MB/s,  46935.1475
%	DDOT1\_OL (300M vector size): 
%	10.5837 s,   10.9330
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4585.2189 MB/s,  4447.2125
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4508.1339 MB/s. 4366.3966
%	$b_\mathrm{MEM}= 45429.6613 MB/s,   
%	vecSUM\_nOL (300M vector size): 
%	10.3444 |   10.3515 ,  10.3879 |   10.3668 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4692.0762 | 4687.7948  MB/s, 4671.4681 | 4681.7738 
%	$b_\mathrm{L2 \rightleftarrows L3}$=  4620.6260 | 4618.3031 MB/s, 4600.5488 | 4612.4519 
%	$b_\mathrm{MEM}= 47039.3017 MB/s,  46879.8278 
%	vecSUM\_OL (300M vector size): 
%	10.7883 s
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4505.8721 MB/s, 
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4434.3056 MB/s.
%	$b_\mathrm{MEM}= 44687.9695 MB/s, 

	&\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white}DDOT4+VectorSUM 
	& \multirow{5}{*}{--} 
	& \multirow{5}{*}{--} %2.3 Emmy 
	& 2.2 &
	\hspace{0.65cm}	-3+0+0
	\multirow{1}{*}{\begin{tikzpicture}[baseline=(current bounding box.east)]
		\draw [thick, red,decorate,decoration={brace,amplitude=10pt,mirror},rotate=90,xshift=-20pt,yshift=12pt](0,0) -- (2,0) node[black,midway,rotate=90,yshift=-0.6cm] {\footnotesize $\pmb{\delta R}$};	
		\end{tikzpicture}}
	& \multirow{5}{*}{--}   & 1.4$\downarrow$ &  12$\downarrow$  
	& 9.96$\downarrow$ & 7.7$\downarrow$   \\ 
	\cline{9-10}\cline{11-12}
%	DDOT4\_nOL (300M vector size): 
%	 43.7386 |   43.7826 s
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4477.4670 | 4475.1615 MB/s
%	$b_\mathrm{L2 \rightleftarrows L3}$=  4428.9273 | 4423.6529 MB/s, 
%	$b_\mathrm{MEM}= 44489.5653 MB/s.
%	DDOT4\_OL (300M vector size): 
%	44.4482 s
%	$b_\mathrm{L1 \rightleftarrows L2}$=  4412.4815 MB/s, 
%	$b_\mathrm{L2 \rightleftarrows L3}$=  4360.8324  MB/s. 
%	$b_\mathrm{MEM}= 44219.4624 MB/s. 
%	vecSUM\_nOL (300M vector size): 
%	10.4142 |   10.2131
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4660.5021 | 4751.1296 MB/s,  
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4588.8229 | 4672.4239 MB/s, 
%	$b_\mathrm{MEM}= 46787.2228 MB/s.
%	vecSUM\_OL (300M vector size): 
%	 11.8449 
%	$b_\mathrm{L1 \rightleftarrows L2}$=  4104.2599 MB/s, 
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4030.3665  MB/s,
%	$b_\mathrm{MEM}=  42307.6355  MB/s.

	&\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white}DDOT3+VectorSUM &   & %1.6 Emmy
	& 2.2 
	& -2+0+0 & & -- &  6 $\downarrow$ 
	& 5.6 $\uparrow$ &  6.7$\downarrow$  \\ 

	\cline{9-10}\cline{11-12}
%	DDOT3\_nOL (300M vector size): 
%	     32.1640 |   32.2785
%	$b_\mathrm{L1 \rightleftarrows L2}$=  4549.6548 | 4529.3544  MB/s
%	$b_\mathrm{L2 \rightleftarrows L3}$=  4508.4576 | 4491.9026 MB/s, 
%	$b_\mathrm{MEM}=  45241.8137  MB/s.
%	DDOT3\_OL (300M vector size): 
%	 32.2535
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4540.9948 MB/s, 
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4499.1225  MB/s.
%	$b_\mathrm{MEM}= 44852.0753  MB/s. 
%	vecSUM\_nOL (300M vector size): 
%	10.3892 |   10.3744
%	$b_\mathrm{L1 \rightleftarrows L2}$=  4671.7096 | 4677.4082  MB/s,  
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4600.6055 | 4605.4812 MB/s, 
%	$b_\mathrm{MEM}= 46834.7032 MB/s.
%	vecSUM\_OL (300M vector size): 
%	11.0822
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4386.4680 MB/s, 
%	$b_\mathrm{L2 \rightleftarrows L3}$=  4309.2662  MB/s,
%	$b_\mathrm{MEM}=  44353.5524 MB/s.	


	&\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white}DDOT+VectorSUM &  &  %1.6 Emmy
	& 1.9
	 & -1+0+0 &   &9.6$\uparrow$ &  17.5$\downarrow$  & 4.42$\uparrow$ & 4.6$\downarrow$  \\ 

	\cline{9-10}\cline{11-12}
%	DDOT\_nOL (300M vector size): 
%	21.8246 |   21.8910 ,  21.1204 |   21.1261, 21.1489 |   21.1897
%	$b_\mathrm{L1 \rightleftarrows L2}$=  4457.0939 | 4440.8749 , 4601.3112 | 4599.1671, 4594.3119 | 4586.2020
%	$b_\mathrm{L2 \rightleftarrows L3}$=  4410.2732 | 4388.1559, 4554.6028 | 4551.2616 ,  4548.4096 | 4539.8708 
%	$b_\mathrm{MEM}= 44630.4255  MB/s, 45935.6083
%	DDOT\_OL (300M vector size): 
%	19.9163   s,  / 19.9533 /  19.9017 / 19.8939 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4882.7463  MB/s,  /4874.4619 / 4884.5979 /  4888.3835 
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4821.5321  MB/s. /4813.3086 / 4817.5307/  4826.2456 
%	$b_\mathrm{MEM}= 44737.1464  MB/s /44729.9827
%	vecSUM\_nOL (300M vector size): 
%	10.5222 |   10.5224,   10.3020 |   10.5675
%	$b_\mathrm{L1 \rightleftarrows L2}$=  4612.5063 | 4611.5720, 4710.4246 | 4592.6306
%	$b_\mathrm{L2 \rightleftarrows L3}$=  4533.2431 | 4531.9530, 4631.5993 | 4510.2944, 46447.3402
%	$b_\mathrm{MEM}= 46260.5425  MB/s. 46447.3402
%	vecSUM\_OL (300M vector size): 
%	12.7741 /  12.9183 /  12.7953 /  12.6220
%	$b_\mathrm{L1 \rightleftarrows L2}$= 3799.9976 MB/s,  3758.0038, 3800.3777, 3851.4684 
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3735.6981  MB/s,  3695.4938,  3735.8253 , 3783.8940
%	$b_\mathrm{MEM}=45256 MB/s,  43467.1302,  43925.5273

	&\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white}DDOT4+DDOT3  & & %1.6 Emmy
	& --
 	& -1+0+0 &    &  5$\downarrow$ & 9.6 $\uparrow$ 
	& 3.2$\downarrow$ & 4.2 $\uparrow$  \\ 

	\cline{9-10}\cline{11-12}
%	DDOT3\_nOL (300M vector size): 
%	31.8938 |   32.0325 s,  31.6281 |   30.5864
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4587.8893 | 4560.9265 MB/s, 4626.4248 | 4777.2421
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4546.5660 | 4523.5800 MB/s, 4582.4740 | 4730.2692
%	$b_\mathrm{MEM}=  45169.8720 MB/s, 44891.7300.
%	DDOT3\_OL (300M vector size): 
%	 25.9560 /  24.3564 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 5635.8279  MB/s, /6007.7506
%	$b_\mathrm{L2 \rightleftarrows L3}$= 5563.4450 MB/s.  / 5926.0623
%	DDOT4\_nOL (300M vector size): 
%	43.5369 |   42.6577 s /  38.2014 |   38.2355
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4520.7762 | 4608.2097 MB/s,  
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4448.8300 | 4541.1719 MB/s, 
%	$b_\mathrm{MEM}=  43323.8116 MB/s.
%	DDOT4\_OL (300M vector size): 
%	 45.7822  s /   
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4299.3924  MB/s, / 
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4229.5078  MB/s, /  
%	$b_\mathrm{MEM}=  41789.4500   MB/s /  

	\multirow{-14}{*}{\rotatebox{90}{\pmb{Same $b_s$}}}
	&\multirow{-6}{*}{\rotatebox{90}{Read-only}}
	&\cellcolor{Cyan!10!white}DDOT3+DDOT &  
	& %1.2 Emmy 
	& --
	& -1+0+0 &   &  11$\downarrow$ & 3$\uparrow$  
	& 1.6$\uparrow$ & 6$\downarrow$ \\ 

%	DDOT3\_nOL (300M vector size): 
%	 32.9910 |   32.9139  / 33.3981 |   32.9666
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4445.5230 | 4457.3078  MB/s / 4394.6182 | 4451.6266
%	$b_\mathrm{L2 \rightleftarrows L3}$=  4397.9648 | 4408.3975 MB/s, / 4333.6094 | 4391.2922
%	$b_\mathrm{MEM}=  44445.8906 MB/s. / 43974.7886
%	DDOT3\_OL (300M vector size): 
%	 37.0423 / 37.0766 /  37.3633 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 3966.0472 MB/s, / 3962.6380 / 3929.3381 
%	$b_\mathrm{L2 \rightleftarrows L3}$=  3916.1854 MB/s.  /  3911.4179/ 3883.9908
%	$b_\mathrm{MEM}= 43566.4712 MB/s. /  43546.3990 /43725.2842
%	DDOT\_nOL (300M vector size): 
%	22.7334 |   22.7862 /  22.7127 |   22.7801 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4277.3704 | 4268.1296 MB/s,  / 4282.4651 | 4267.3890
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4230.8384 | 4221.4381 MB/s, / 4237.6408 | 4216.7168
%	$b_\mathrm{MEM}= 43176.0500  MB/s. / 43157.0754
%	DDOT\_OL (300M vector size): 
%	22.0839 /  22.4020 / 20.5444 / 20.4746 / 22.0515 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4401.9191 MB/s, / 4340.3708 / 4732.0053 / 4748.6827 / 4410.0286
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4343.6104  MB/s. / 4283.9591 / 4656.1023 / 4673.8340 / 4357.1131

	\cmidrule[1.5pt]{1-11}
	&
	&\cellcolor{Cyan!10!white}Schoenauer+vectorSUM 
	& \multirow{2}{*}{-5.95}
	& \multirow{2}{*}{5} &  3 
	&
\hspace{0.65cm} -2-1-1
\multirow{1}{*}{\begin{tikzpicture}[baseline=(current bounding box.east)]
	\draw [thick, red,decorate,decoration={brace,amplitude=10pt,mirror},rotate=90,xshift=-20pt,yshift=12pt](0,0) -- (0.8,0) node[black,midway,rotate=90,yshift=-0.6cm] {\footnotesize $\pmb{\delta R}$};
	\end{tikzpicture}}
 	& \multirow{2}{*}{$\div$2}
 	& 17$\uparrow$ &  22$\downarrow$ 
 	& 1.77 $\uparrow$ &  20.5$\downarrow$\\  
	\cline{9-10}\cline{11-12}
%	24 / vecSUM\_nOL (300M vector size): 
%	10.3613 |   10.3556 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$=  4684.3221 | 4685.8987 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$=  4613.0461 | 4614.0112 MB/s,
%	$b_\mathrm{MEM}= 46934 MB/s.
%	24 / vecSUM\_OL (300M vector size): 
%	13.2748    s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 3663.7158  MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$=  3603.3663 MB/s.
%	Schoenauer\_nOL (300M vector size): 
%	59.0315 |   59.0685 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4119.9243 | 4116.7565  MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4082.1967 | 4080.4488   MB/s,
%	$b_\mathrm{MEM}= 41202(32935+8267) MB/s.
%	Schoenauer\_OL (300M vector size): 
%	 50.3527 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4827.7120 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$=  4787.5995   MB/s.		


	 &\cellcolor[gray]{0.9}
	&\cellcolor{Cyan!10!white}Schoenauer+DDOT  & &  & 1.2 &
	-1-1-1
	& & 8$\uparrow$ &  14$\downarrow$ 
	& 1.63$\downarrow$ & 15.8$\downarrow$  \\ 
	\cline{4-11}
%	DDOT\_nOL (300M vector size): 
%	21.5008 |   21.8716 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4522.8792 | 4447.2473 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4475.9528 | 4401.4795 MB/s,
%	$b_\mathrm{MEM}= 44965 MB/s.
%	DDOT\_OL (300M vector size): 
%	24.9142   s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 3903.6319 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3858.1200 MB/s.
%	Schoenauer\_nOL (300M vector size): 
%	58.2204 |   58.1918 | s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$=  4175.9100 | 4178.1832  MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$=  4138.4898 | 4140.3313 MB/s,
%	$b_\mathrm{MEM}= 41687(33354+8332) MB/s.
%	Schoenauer\_OL (300M vector size): 
%	53.8569 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4515.9124 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4475.3448  MB/s,
%	$b_\mathrm{MEM}= 42467(37901+4565) MB/s.
	
	 &\cellcolor[gray]{0.9}
	&\cellcolor{Cyan!10!white}ADD+vectorSUM  
	& \multirow{5}{*}{-7.4 }
	& \multirow{5}{*}{5.8} 
	& 5.1
	&
	\hspace{0.65cm} -1-1-1
	\multirow{1}{*}{\begin{tikzpicture}[baseline=(current bounding box.east)]
		\draw [thick, red,decorate,decoration={brace,amplitude=10pt,mirror},rotate=90,xshift=-20pt,yshift=12pt](0,0) -- (2,0) node[black,midway,rotate=90,yshift=-0.6cm] {\footnotesize $\pmb{\delta R}$};	
		\end{tikzpicture}}
	& $\div$3 & 22$\uparrow$ &  25$\downarrow$ & 18$\uparrow$ & 22.6$\downarrow$ \\  
	\cline{9-10}\cline{11-12}
%	ADD\_nOL (300M vector size): 
%	96/ 47.9071 |   47.9585  s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4053.1322 | 4049.6077 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4012.1315 | 4007.2858 MB/s,
%	$b_\mathrm{MEM}=40605(30435+10169) MB/s.
%	ADD\_OL (300M vector size): 
%	96/ 39.3860 s,  22%
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4930.3349 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4885.2608 MB/s.
%	vectorSUM\_nOL (300M vector size): 
%	24/ 10.3924 |   10.3654 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$=  4669.2078 | 4682.4786 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$=   4598.2260 | 4610.0230 MB/s,
%	$b_\mathrm{MEM}=46847 MB/s.
%	vectorSUM\_OL (300M vector size): 
%	24 /13.8273  s, 25 %
%	$b_\mathrm{L1 \rightleftarrows L2}$= 3516.7278 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3456.6615 MB/s,
%	$b_\mathrm{MEM}= 41816(35715+6100) MB/s.
 	&\cellcolor[gray]{0.9}
	&\cellcolor{Cyan!10!white}WAXPBY+DDOT &  &  & 3.2 &
	0-1-1 & 
	\hspace{1cm} --
	\multirow{1}{*}{\begin{tikzpicture}[baseline=(current bounding box.east)]
		\draw [thick, red,decorate,decoration={brace,amplitude=10pt,mirror},rotate=90,xshift=-20pt,yshift=12pt](0,0) -- (0.75,0) node[black,midway,rotate=90,yshift=-0.6cm] {\footnotesize $\pmb{\delta B_c}$};	
		\end{tikzpicture}}
	 & 15$\uparrow$    & 19$\downarrow$& 14.5$\uparrow$ & 18$\downarrow$ \\ 	
	 \cline{9-10}\cline{11-12}
%	WAXPBY\_nOL (300M vector size): 
%	96.03 / 47.5771 |   47.5505 s,  47.4130 |   47.4089, 40.7422 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4080.9790 | 4082.3280 MB/s, 4094.1965 | 4095.8068  MB/s, 4767.3351
%	$b_\mathrm{L2 \rightleftarrows L3}$=   4034.4211 | 4038.8822 MB/s,4050.3670 | 4049.3124, 4713.0476 
%	$b_\mathrm{MEM}= 40941(30708+10233) MB/s. 40456.3841
%	WAXPBY\_OL (300M vector size): 
%	96.03 / 40.5934  s, 42.1623  
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4784.7842  MB/s,  4604.0201
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4733.2915 MB/s.  4556.2679
%	$b_\mathrm{MEM}=42638(36601+6037) MB/s.
%	48 / DDOT\_nOL (300M vector size): 
%	21.5591 |   21.6369 s, 21.1799 |   21.2036 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4511.6891 | 4493.2738 MB/s,  4587.0719 | 4583.6051
%	$b_\mathrm{L2 \rightleftarrows L3}$=  4465.5427 | 4442.9733  MB/s,  4538.7459 | 4536.8177
%	$b_\mathrm{MEM}=45128 MB/s.
%	48 / DDOT\_OL (300M vector size): 
%	26.7727  s,  26.0724
%	$b_\mathrm{L1 \rightleftarrows L2}$= 3633.2082 MB/s,  3728.8474
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3597.7453 MB/s,  3689.5714

% Meggie
%	WAXPBY\_nOL (300M vector size): 
%	36.7292 s, 36.7718 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 5286.3976 MB/s, 5280.3594
%	$b_\mathrm{L2 \rightleftarrows L3}$= 5253.9102  MB/s, 5247.7940
%	$b_\mathrm{MEM}=  52890.8781 MB/s. 52901.9787
%	WAXPBY\_OL (300M vector size): 
%	s
%	$b_\mathrm{L1 \rightleftarrows L2}$=MB/s, 
%	$b_\mathrm{L2 \rightleftarrows L3}$= MB/s.  
%	$b_\mathrm{MEM}= MB/s.
%	DDOT\_nOL (300M vector size): 
%	s
%	$b_\mathrm{L1 \rightleftarrows L2}$=  MB/s, 
%	$b_\mathrm{L2 \rightleftarrows L3}$=   MB/s,
%	$b_\mathrm{MEM}= MB/s.
%	DDOT\_OL (300M vector size): 
%	s
%	$b_\mathrm{L1 \rightleftarrows L2}$= MB/s,  
%	$b_\mathrm{L2 \rightleftarrows L3}$= MB/s,  
%	$b_\mathrm{MEM}= MB/s.

	&\cellcolor[gray]{0.9}
	&\cellcolor{Cyan!10!white}ADD+DDOT  & & & 3.2& 0-1-1 & 
	$\div$3
	&15$\uparrow$ &  19$\downarrow$ 
	& 14.5$\uparrow$ & 18$\downarrow$\\ 	
	\cline{9-10}\cline{11-12}
%	ADD\_nOL (300M vector size): 
%	96/ 47.5018 |   47.4912 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$=  4086.7004 | 4086.8102 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4043.5477 | 4046.2284 MB/s,
%	$b_\mathrm{MEM}=40890(30675+10215) MB/s.
%	ADD\_OL (300M vector size): 
%	96/ 41.2539 s, 15%
%	$b_\mathrm{L1 \rightleftarrows L2}$=  4706.6871  MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4661.8406 MB/s.
%	DDOT\_nOL (300M vector size): 
%	 21.5343 |   21.7443 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$=  4515.4278 | 4470.6565 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$=  4464.0021 | 4419.3048 MB/s,
%	$b_\mathrm{MEM}=45039 MB/s.
%	DDOT\_OL 3005M vector size): 
%	 26.6543  s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 3649.5528 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3609.0345 MB/s. 


	&\cellcolor[gray]{0.9}
	&\cellcolor{Cyan!10!white}ADD+DDOT3 & & & 3 & 1-1-1  &$\div$3& 18.9$\uparrow$ &  18.2$\downarrow$ 
	& 13.11$\uparrow$ & 16.8$\downarrow$\\  	
	\cline{9-10}\cline{11-12}

%	DDOT3: s+=a[i]*b[i]*c[i]
%%	ADD\_nOL (300M vector size):
%|           Runtime (RDTSC) [s]          |    47.4938 |   47.5412 |
%|          Runtime unhalted [s]          |    46.9548 |   47.0198 |
%|               Clock [MHz]              |  2199.5550 | 2199.7891 |
%|                   CPI                  |     8.4922 |    8.6571 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  3065.7238 | 3062.7299 |
%|   L2 to L1 load data volume [GBytes]   |   145.6028 |  145.6058 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1020.7525 | 1020.6666 |
%|   L1 to L2 evict data volume [GBytes]  |    48.4794 |   48.5237 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  4086.4763 | 4083.3965 |
%|   L1 to/from L2 data volume [GBytes]   |   194.0821 |  194.1295 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  3052.6082 | 3049.9571 |
%|   L3 to L2 load data volume [GBytes]   |   144.9798 |  144.9986 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |   992.9871 |  990.9037 |
%|   L2 to L3 evict data volume [GBytes]  |    47.1607 |   47.1087 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  4045.5953 | 4040.8609 |
%|   L2 to/from L3 data volume [GBytes]   |   192.1405 |  192.1073 |
%|    System to L3 bandwidth [MBytes/s]   |     nan    |    nan    |
%|    System to L3 data volume [GBytes]   |     nan    |    nan    |
%|    L3 to memory bandwidth [MBytes/s]   |          0 |         0 |
%|    L3 to memory data volume [GBytes]   |          0 |         0 |
%| L3 to/from system bandwidth [MBytes/s] |     nan    |    nan    |
%| L3 to/from system data volume [GBytes] |     nan    |    nan    |
%|    Memory read bandwidth [MBytes/s]    | 30734.1845 |         0 |
%|    Memory read data volume [GBytes]    |  1459.6820 |         0 |
%|    Memory write bandwidth [MBytes/s]   | 10253.8937 |         0 |
%|    Memory write data volume [GBytes]   |   486.9960 |         0 |
%|       Memory bandwidth [MBytes/s]      | 40988.0783 |         0 |
%|       Memory data volume [GBytes]      |  1946.6780 |         0 |
%%	ADD\_OL (300M vector size):
%%	39.9481  s, 
%%	$b_\mathrm{L1 \rightleftarrows L2}$= 4858.9536  MB/s,
%%	$b_\mathrm{L2 \rightleftarrows L3}$= 4811.9840  MB/s.
%%	DDOT3\_nOL (300M vector size): 
%|           Runtime (RDTSC) [s]          |    32.3730 |   32.2928 |
%|          Runtime unhalted [s]          |    31.9709 |   31.9133 |
%|               Clock [MHz]              |  2199.5561 | 2199.7887 |
%|                   CPI                  |     5.7228 |    5.8675 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  4516.5054 | 4527.9802 |
%|   L2 to L1 load data volume [GBytes]   |   146.2131 |  146.2212 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |     3.4754 |    4.5340 |
%|   L1 to L2 evict data volume [GBytes]  |     0.1125 |    0.1464 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  4519.9808 | 4532.5142 |
%|   L1 to/from L2 data volume [GBytes]   |   146.3256 |  146.3677 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  4475.9324 | 4486.9120 |
%|   L3 to L2 load data volume [GBytes]   |   144.8996 |  144.8950 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |     3.3874 |    4.2015 |
%|   L2 to L3 evict data volume [GBytes]  |     0.1097 |    0.1357 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  4479.3198 | 4491.1135 |
%|   L2 to/from L3 data volume [GBytes]   |   145.0092 |  145.0307 |
%|    System to L3 bandwidth [MBytes/s]   |     nan    |    nan    |
%|    System to L3 data volume [GBytes]   |     nan    |    nan    |
%|    L3 to memory bandwidth [MBytes/s]   |          0 |         0 |
%|    L3 to memory data volume [GBytes]   |          0 |         0 |
%| L3 to/from system bandwidth [MBytes/s] |     nan    |    nan    |
%| L3 to/from system data volume [GBytes] |     nan    |    nan    |
%|    Memory read bandwidth [MBytes/s]    | 45106.8330 |         0 |
%|    Memory read data volume [GBytes]    |  1460.2458 |         0 |
%|    Memory write bandwidth [MBytes/s]   |    59.9871 |         0 |
%|    Memory write data volume [GBytes]   |     1.9420 |         0 |
%|       Memory bandwidth [MBytes/s]      | 45166.8201 |         0 |
%|       Memory data volume [GBytes]      |  1462.1877 |         0 |
%%	DDOT3\_OL (300M vector size): 
%%	40.0153 s, 
%%	$b_\mathrm{L1 \rightleftarrows L2}$= 3659.7105 MB/s,
%%	$b_\mathrm{L2 \rightleftarrows L3}$= 3625.7005 MB/s.


	&\cellcolor[gray]{0.9}
	&\cellcolor{Cyan!10!white}ADD+DDOT4 &  & & 2.9 &
	 2-1-1
 &$\div$3
 & 31.4$\uparrow$ &  27.1$\downarrow$ 
 & 17$\uparrow$ & 23.4$\downarrow$ \\  
	\cline{4-11}
%%	DDOT4: s+=a[i]*b[i]*c[i]*d[i]
%%%	ADD\_nOL (300M vector size):
%|           Runtime (RDTSC) [s]          |    47.6082 |   47.6141 |
%|          Runtime unhalted [s]          |    47.0495 |   47.0836 |
%|               Clock [MHz]              |  2200.0029 | 2199.7943 |
%|                   CPI                  |     8.3936 |    8.5768 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  3058.4021 | 3057.8519 |
%|   L2 to L1 load data volume [GBytes]   |   145.6049 |  145.5969 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1019.3516 | 1018.2224 |
%|   L1 to L2 evict data volume [GBytes]  |    48.5295 |   48.4817 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  4077.7537 | 4076.0742 |
%|   L1 to/from L2 data volume [GBytes]   |   194.1344 |  194.0786 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  3045.3408 | 3045.0597 |
%|   L3 to L2 load data volume [GBytes]   |   144.9831 |  144.9878 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |   989.1081 |  990.9658 |
%|   L2 to L3 evict data volume [GBytes]  |    47.0896 |   47.1839 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  4034.4489 | 4036.0254 |
%|   L2 to/from L3 data volume [GBytes]   |   192.0727 |  192.1717 |
%|    System to L3 bandwidth [MBytes/s]   |     nan    |    nan    |
%|    System to L3 data volume [GBytes]   |     nan    |    nan    |
%|    L3 to memory bandwidth [MBytes/s]   |          0 |         0 |
%|    L3 to memory data volume [GBytes]   |          0 |         0 |
%| L3 to/from system bandwidth [MBytes/s] |     nan    |    nan    |
%| L3 to/from system data volume [GBytes] |     nan    |    nan    |
%|    Memory read bandwidth [MBytes/s]    | 30672.9700 |         0 |
%|    Memory read data volume [GBytes]    |  1460.2840 |         0 |
%|    Memory write bandwidth [MBytes/s]   | 10234.0982 |         0 |
%|    Memory write data volume [GBytes]   |   487.2267 |         0 |
%|       Memory bandwidth [MBytes/s]      | 40907.0682 |         0 |
%|       Memory data volume [GBytes]      |  1947.5107 |         0 |
%%%	ADD\_OL (300M vector size):
%%%	36.2253 s, 
%%%	$b_\mathrm{L1 \rightleftarrows L2}$= 5358.1513 MB/s,
%%%	$b_\mathrm{L2 \rightleftarrows L3}$= 5302.1832 MB/s.
%%%	DDOT4\_nOL (300M vector size): 
%|           Runtime (RDTSC) [s]          |    37.1607 |   37.1043 |
%|          Runtime unhalted [s]          |    36.1867 |   36.1658 |
%|               Clock [MHz]              |  2199.9993 | 2199.7921 |
%|                   CPI                  |     4.3561 |    4.3948 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  5271.2606 | 5279.5235 |
%|   L2 to L1 load data volume [GBytes]   |   195.8838 |  195.8929 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |     6.3405 |    5.9315 |
%|   L1 to L2 evict data volume [GBytes]  |     0.2356 |    0.2201 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  5277.6011 | 5285.4549 |
%|   L1 to/from L2 data volume [GBytes]   |   196.1195 |  196.1129 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  5205.8479 | 5213.5697 |
%|   L3 to L2 load data volume [GBytes]   |   193.4531 |  193.4457 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |     4.6815 |    3.9142 |
%|   L2 to L3 evict data volume [GBytes]  |     0.1740 |    0.1452 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  5210.5294 | 5217.4838 |
%|   L2 to/from L3 data volume [GBytes]   |   193.6270 |  193.5909 |
%|    System to L3 bandwidth [MBytes/s]   |     nan    |    nan    |
%|    System to L3 data volume [GBytes]   |     nan    |    nan    |
%|    L3 to memory bandwidth [MBytes/s]   |          0 |         0 |
%|    L3 to memory data volume [GBytes]   |          0 |         0 |
%| L3 to/from system bandwidth [MBytes/s] |     nan    |    nan    |
%| L3 to/from system data volume [GBytes] |     nan    |    nan    |
%|    Memory read bandwidth [MBytes/s]    | 39630.5432 |         0 |
%|    Memory read data volume [GBytes]    |  1472.6995 |         0 |
%|    Memory write bandwidth [MBytes/s]   |    69.5365 |         0 |
%|    Memory write data volume [GBytes]   |     2.5840 |         0 |
%|       Memory bandwidth [MBytes/s]      | 39700.0798 |         0 |
%|       Memory data volume [GBytes]      |  1475.2835 |         0 |
%%%	DDOT4\_OL (300M vector size): 
%%%	 50.9162  s, 
%%%	$b_\mathrm{L1 \rightleftarrows L2}$= 3849.1102 MB/s,
%%%	$b_\mathrm{L2 \rightleftarrows L3}$= 3804.8797 MB/s.	

	
	 &\cellcolor[gray]{0.9}
	 &\cellcolor{Cyan!10!white}DCOPY+vectorSUM  
	& \multirow{4}{*}{-9.1}
	& \multirow{4}{*}{5.9}  
	& 4.8 (8.3\%)
	&
	 \hspace{0.65cm} 0-1-1
	 \multirow{1}{*}{\begin{tikzpicture}[baseline=(current bounding box.east)]
	 	\draw [thick, red,decorate,decoration={brace,amplitude=10pt,mirror},rotate=90,xshift=-20pt,yshift=12pt](0,0) -- (1.7,0) node[black,midway,rotate=90,yshift=-0.6cm] {\footnotesize $\pmb{\delta R }$};	
	 	\end{tikzpicture}}
	  & \multirow{4}{*}{$\div$2} & 25.5$\uparrow$ &  30.5$\downarrow$  & 21.1$\uparrow$ & 26$\downarrow$\\ \cline{9-10}\cline{11-12}
%	DCOPY\_nOL (300M vector size): 
%	 36.1109 |   36.1633 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4030.2177 | 4023.8048 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3960.5790 | 3956.5149 MB/s,
%	$b_\mathrm{MEM}=(+) MB/s.
%	DCOPY\_OL (300M vector size): 
%	28.7894 s,
%	$b_\mathrm{L1 \rightleftarrows L2}$=  5054.7485 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4974.6283 MB/s.
%	vectorSUM\_nOL (300M vector size): 
%	10.3784 |   10.3711 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4676.5647 | 4678.8098 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4604.7447 | 4606.1381 MB/s,
%	$b_\mathrm{MEM}=46868 MB/s.
%	vectorSUM\_OL (300M vector size): 
%	14.9513 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 3253.5746 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3197.6678 MB/s,
%	$b_\mathrm{MEM}=41214 MB/s.	

	 &\cellcolor[gray]{0.9}
	 &\cellcolor{Cyan!10!white}DCOPY+DDOT &  & & 3 & 1-1-1  &  & 21.5$\uparrow$ &  22$\downarrow$ 
	 & 17.33$\uparrow$  &  21.6$\downarrow$ \\ \cline{9-10}\cline{11-12}
%	DDOT\_nOL (300M vector size): 
%	21.5064 |   21.5898 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 4522.8411 | 4503.6523 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 4476.4443 | 4455.2108   MB/s,
%	$b_\mathrm{MEM}= 45198 MB/s.
%	DDOT\_OL (300M vector size): 
%	27.5833  s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 3527.9396  MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 3496.6061 MB/s.
%	DCOPY\_nOL (300M vector size): 
%	25.8745 |   25.8489 s, 
%	$b_\mathrm{L1 \rightleftarrows L2}$=  5613.8084 | 5618.9825  MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$=  5435.9399 | 5451.0586 MB/s,
%	$b_\mathrm{MEM}= 37578(18835+18742) MB/s.
%	DCOPY\_OL (300M vector size): 
%	21.4691 
%	$b_\mathrm{L1 \rightleftarrows L2}$= 6769.8556 MB/s,
%	$b_\mathrm{L2 \rightleftarrows L3}$= 6576.0132  MB/s,
%	$b_\mathrm{MEM}= 40276(28927+11349) MB/s.

	 &\cellcolor[gray]{0.9}
	 &\cellcolor{Cyan!10!white}DCOPY+DDOT3 & & & 2.7 & 2-1-1  &  & 23.6$\uparrow$ &  26.5$\downarrow$ 
	 & 15.5$\uparrow$ & 20$\downarrow$ \\  \cline{9-10}\cline{11-12}

%%	DDOT3: s+=a[i]*b[i]*c[i]
%%%	DCOPY\_nOL (300M vector size):
%|           Runtime (RDTSC) [s]          |    35.7984 |   35.8279 |
%|          Runtime unhalted [s]          |    35.3852 |   35.4394 |
%|               Clock [MHz]              |  2200.0021 | 2199.9987 |
%|                   CPI                  |    11.0652 |   11.2450 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  2709.3603 | 2707.1989 |
%|   L2 to L1 load data volume [GBytes]   |    96.9907 |   96.9933 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1353.2490 | 1352.2960 |
%|   L1 to L2 evict data volume [GBytes]  |    48.4441 |   48.4499 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  4062.6093 | 4059.4949 |
%|   L1 to/from L2 data volume [GBytes]   |   145.4348 |  145.4432 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  2685.0696 | 2683.6999 |
%|   L3 to L2 load data volume [GBytes]   |    96.1211 |   96.1514 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1311.4258 | 1309.8463 |
%|   L2 to L3 evict data volume [GBytes]  |    46.9469 |   46.9291 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  3996.4954 | 3993.5463 |
%|   L2 to/from L3 data volume [GBytes]   |   143.0680 |  143.0804 |
%|    System to L3 bandwidth [MBytes/s]   |     nan    |    nan    |
%|    System to L3 data volume [GBytes]   |     nan    |    nan    |
%|    L3 to memory bandwidth [MBytes/s]   |          0 |         0 |
%|    L3 to memory data volume [GBytes]   |          0 |         0 |
%| L3 to/from system bandwidth [MBytes/s] |     nan    |    nan    |
%| L3 to/from system data volume [GBytes] |     nan    |    nan    |
%|    Memory read bandwidth [MBytes/s]    | 27201.4517 |         0 |
%|    Memory read data volume [GBytes]    |   973.7674 |         0 |
%|    Memory write bandwidth [MBytes/s]   | 13585.3946 |         0 |
%|    Memory write data volume [GBytes]   |   486.3348 |         0 |
%|       Memory bandwidth [MBytes/s]      | 40786.8463 |         0 |
%|       Memory data volume [GBytes]      |  1460.1022 |         0 |
%%%	28.9638   s, 
%%%	$b_\mathrm{L1 \rightleftarrows L2}$= 5021.3752   MB/s,
%%%	$b_\mathrm{L2 \rightleftarrows L3}$=  4939.1925  MB/s.
%%%	DDOT3\_nOL (300M vector size): 
%|           Runtime (RDTSC) [s]          |    32.2396 |   32.2778 |
%|          Runtime unhalted [s]          |    31.8526 |   31.8989 |
%|               Clock [MHz]              |  2200.0021 | 2199.9989 |
%|                   CPI                  |     5.9121 |    5.9719 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  4535.1745 | 4530.1328 |
%|   L2 to L1 load data volume [GBytes]   |   146.2120 |  146.2227 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |     3.5786 |    4.4311 |
%|   L1 to L2 evict data volume [GBytes]  |     0.1154 |    0.1430 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  4538.7532 | 4534.5639 |
%|   L1 to/from L2 data volume [GBytes]   |   146.3274 |  146.3657 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  4494.8345 | 4489.2735 |
%|   L3 to L2 load data volume [GBytes]   |   144.9115 |  144.9039 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |     3.4923 |    4.1267 |
%|   L2 to L3 evict data volume [GBytes]  |     0.1126 |    0.1332 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  4498.3268 | 4493.4002 |
%|   L2 to/from L3 data volume [GBytes]   |   145.0241 |  145.0371 |
%|    System to L3 bandwidth [MBytes/s]   |     nan    |    nan    |
%|    System to L3 data volume [GBytes]   |     nan    |    nan    |
%|    L3 to memory bandwidth [MBytes/s]   |          0 |         0 |
%|    L3 to memory data volume [GBytes]   |          0 |         0 |
%| L3 to/from system bandwidth [MBytes/s] |     nan    |    nan    |
%| L3 to/from system data volume [GBytes] |     nan    |    nan    |
%|    Memory read bandwidth [MBytes/s]    | 45196.4898 |         0 |
%|    Memory read data volume [GBytes]    |  1457.1149 |         0 |
%|    Memory write bandwidth [MBytes/s]   |    57.4812 |         0 |
%|    Memory write data volume [GBytes]   |     1.8532 |         0 |
%|       Memory bandwidth [MBytes/s]      | 45253.9709 |         0 |
%|       Memory data volume [GBytes]      |  1458.9681 |         0 |
%%%	DDOT3\_OL (300M vector size): 
%%%	43.8750  s, 
%%%	$b_\mathrm{L1 \rightleftarrows L2}$= 3337.9722 MB/s,
%%%	$b_\mathrm{L2 \rightleftarrows L3}$= 3308.3782 MB/s.
%	

	 \multirow{-11}{*}{\rotatebox{90}{\pmb{Different $b_s$}}}
	 & \multirow{-11}{*}{\rotatebox{90}{Read-write/Read-only}}
	 &\cellcolor{Cyan!10!white}DCOPY+DDOT4 &  &  & 2.6 &
3-1-1
 &  & 19.1$\uparrow$ &  32.4$\downarrow$ 
 & 15$\uparrow$ &  31.6$\downarrow$ \\  

%%	DDOT4: s+=a[i]*b[i]*c[i]*d[i]
%%%	DCOPY\_nOL (300M vector size):
%|           Runtime (RDTSC) [s]          |    35.9543 |   35.9539 |
%|          Runtime unhalted [s]          |    35.5446 |   35.5758 |
%|               Clock [MHz]              |  2199.9209 | 2199.9651 |
%|                   CPI                  |    10.8868 |   11.3078 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  2697.5946 | 2697.7143 |
%|   L2 to L1 load data volume [GBytes]   |    96.9900 |   96.9932 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |  1347.2885 | 1347.5273 |
%|   L1 to L2 evict data volume [GBytes]  |    48.4408 |   48.4488 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  4044.8831 | 4045.2416 |
%|   L1 to/from L2 data volume [GBytes]   |   145.4308 |  145.4420 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  2673.1778 | 2674.2407 |
%|   L3 to L2 load data volume [GBytes]   |    96.1121 |   96.1492 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |  1305.8223 | 1305.4933 |
%|   L2 to L3 evict data volume [GBytes]  |    46.9499 |   46.9375 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  3979.0001 | 3979.7340 |
%|   L2 to/from L3 data volume [GBytes]   |   143.0620 |  143.0868 |
%|    System to L3 bandwidth [MBytes/s]   |     nan    |    nan    |
%|    System to L3 data volume [GBytes]   |     nan    |    nan    |
%|    L3 to memory bandwidth [MBytes/s]   |          0 |         0 |
%|    L3 to memory data volume [GBytes]   |          0 |         0 |
%| L3 to/from system bandwidth [MBytes/s] |     nan    |    nan    |
%| L3 to/from system data volume [GBytes] |     nan    |    nan    |
%|    Memory read bandwidth [MBytes/s]    | 27095.4040 |         0 |
%|    Memory read data volume [GBytes]    |   974.1952 |         0 |
%|    Memory write bandwidth [MBytes/s]   | 13532.0109 |         0 |
%|    Memory write data volume [GBytes]   |   486.5334 |         0 |
%|       Memory bandwidth [MBytes/s]      | 40627.4149 |         0 |
%|       Memory data volume [GBytes]      |  1460.7286 |         0 |
%%%	DCOPY\_OL (300M vector size):
%%%	29.0766  s, 
%%%	$b_\mathrm{L1 \rightleftarrows L2}$= 5001.9302  MB/s,
%%%	$b_\mathrm{L2 \rightleftarrows L3}$= 4921.5703   MB/s.
%%%	DDOT4\_nOL (300M vector size): 
%|           Runtime (RDTSC) [s]          |    43.4472 |   43.5912 |
%|          Runtime unhalted [s]          |    42.9008 |   43.0568 |
%|               Clock [MHz]              |  2199.9209 | 2199.9649 |
%|                   CPI                  |     5.6145 |    5.6022 |
%|   L2 to L1 load bandwidth [MBytes/s]   |  4501.0595 | 4486.3898 |
%|   L2 to L1 load data volume [GBytes]   |   195.5587 |  195.5673 |
%|   L1 to L2 evict bandwidth [MBytes/s]  |     3.6366 |    4.4810 |
%|   L1 to L2 evict data volume [GBytes]  |     0.1580 |    0.1953 |
%|   L1 to/from L2 bandwidth [MBytes/s]   |  4504.6960 | 4490.8709 |
%|   L1 to/from L2 data volume [GBytes]   |   195.7167 |  195.7626 |
%|   L3 to L2 load bandwidth [MBytes/s]   |  4454.9633 | 4440.1068 |
%|   L3 to L2 load data volume [GBytes]   |   193.5559 |  193.5498 |
%|   L2 to L3 evict bandwidth [MBytes/s]  |     3.5266 |    4.2171 |
%|   L2 to L3 evict data volume [GBytes]  |     0.1532 |    0.1838 |
%|   L2 to/from L3 bandwidth [MBytes/s]   |  4458.4899 | 4444.3239 |
%|   L2 to/from L3 data volume [GBytes]   |   193.7091 |  193.7336 |
%|    System to L3 bandwidth [MBytes/s]   |     nan    |    nan    |
%|    System to L3 data volume [GBytes]   |     nan    |    nan    |
%|    L3 to memory bandwidth [MBytes/s]   |          0 |         0 |
%|    L3 to memory data volume [GBytes]   |          0 |         0 |
%| L3 to/from system bandwidth [MBytes/s] |     nan    |    nan    |
%| L3 to/from system data volume [GBytes] |     nan    |    nan    |
%|    Memory read bandwidth [MBytes/s]    | 44661.6260 |         0 |
%|    Memory read data volume [GBytes]    |  1940.4248 |         0 |
%|    Memory write bandwidth [MBytes/s]   |    51.6462 |         0 |
%|    Memory write data volume [GBytes]   |     2.2439 |         0 |
%|       Memory bandwidth [MBytes/s]      | 44713.2723 |         0 |
%|       Memory data volume [GBytes]      |  1942.6687 |         0 |
%%%	DDOT4\_OL (300M vector size): 
%%%	57.5665  s, 
%%%	$b_\mathrm{L1 \rightleftarrows L2}$= 3402.1417  MB/s,
%%%	$b_\mathrm{L2 \rightleftarrows L3}$= 3368.2572 MB/s.
%

	\specialrule{2.5pt}{1pt}{1pt}
\end{tabular*}


==> tables/tab6_HPCG.tex <==
\setlength\tabcolsep{0pt}
\setlength\extrarowheight{0pt} 
%\def\arraystretch{1.25} % vertical stretch factor
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}cllcccc}
	%\begin{tabular}[fragile]{|l|l|c|c|c|c|}
	\specialrule{2.5pt}{1pt}{1pt}
	\rowcolor[gray]{0.9}
	& {Computation} & {Pseudo-code for loop\mbox{$\S$} body} & CL  & {Code-} & \multicolumn{2}{c}{Memory pressure $P_\mathrm{MEM}$} 	\\
%	\cline{6-7}
	\rowcolor[gray]{0.9}
	& {(+communication)} & {of computational kernels} & transfer & {balance $B_c$}  & $\frac{T_\mathrm{L3-MEM}}{T}\cdot 100$ & $T_\mathrm{L3-MEM} : T$  \\
	\rowcolor[gray]{0.9}
	\multirow{-3}{*}{\rotatebox{90}{Algo}}& {kernels} & & (R+W+RFO) & [\si{\bytes\per\F}] & [\%]  & [\si{\cycles\per\iter}]  \\
	
	\specialrule{2.5pt}{1pt}{1pt}
	& \cellcolor{Cyan!10!white}FORWARD-SYMGS  &       a[i] -= (val[i])[j]*b[(id[i])[j]]
	& 5 (3+1+1) &  \hspace{0.25cm} 6.52\mbox{$\ddagger$} 	
	\multirow{1}{*}{\begin{tikzpicture}[baseline=(current bounding box.east)]
	\draw [thick, red,decorate,decoration={brace,amplitude=10pt,mirror},rotate=90,xshift=-20pt,yshift=12pt](0,0) -- (1.15,0) node[black,midway,rotate=90,yshift=-0.6cm] {\footnotesize $\mathbf{10.17}$};	
	\end{tikzpicture}} &  
	\hspace{0.6cm} 40.2
	\multirow{1}{*}{\begin{tikzpicture}[baseline=(current bounding box.east)]
		\draw [thick, red,decorate,decoration={brace,amplitude=10pt,mirror},rotate=90,xshift=-20pt,yshift=12pt](0,0) -- (1.15,0) node[black,midway,rotate=90,yshift=-0.6cm] {\footnotesize $\mathbf{39.9}$};	
		\end{tikzpicture}}
	& 16.8 : 42.8   \\ 
	& (+HALO-EXCHANGE)  &      a[i] += b[i]*diag[i][0]
	& 2 (2+0+0) & 8 & 33.3 &  6 : 18  \\ 
	\cellcolor[gray]{0.9}&  &      b[i] = a[i]/diag[i][0]
	& 2 (0+1+1) & 16 & 46.2 &  6.87 : 14.87     \\
	\cellcolor[gray]{0.9}& \cellcolor{Cyan!10!white}BACKWARD-SYMGS  &       a[i] -= (val[i])[j]*b[(id[i])[j]]
	&5 (3+1+1) & 6.52 & 40.2 & 16.8 : 42.8    \\ 
	\cellcolor[gray]{0.9}&  &      a[i] += b[i]*diag[i][0]
	& 2 (2+0+0) & 8 & 33.3 &  6 : 18   \\ 
	\cellcolor[gray]{0.9}&  &      b[i] = a[i]/diag[i][0]
	& 2 (0+1+1) & 16   & 46.2 &  6.87 : 14.87      \\ \cline{2-7}
	\cellcolor[gray]{0.9}& \cellcolor{Cyan!10!white}SPMV  & t += (val[i])[j]*b[(id[i])[j]] & 5 (3+1+1) & 6.52 & 40.2 & 16.8 : 42.8     \\ 
	\cellcolor[gray]{0.9}& (+HALO-EXCHANGE)  & c[i] = t & & &    \\ \cline{2-7}
	\cellcolor[gray]{0.9}& \cellcolor{Cyan!10!white}RESTRICTION  &val1[i] = a[op[i]] - val2[op[i]] & 5 (3+1+1) & 36 & 39.6  & 15.12 : 38.12    \\  \cline{2-7}
	\cellcolor[gray]{0.9}& \cellcolor{Cyan!10!white}PROLONGATION  & b[op[i]] += val3[i] & 4 (1+1+2) & 28 &  42.8  & 12 : 28    \\  \cline{2-7}
	\cellcolor[gray]{0.9}& \cellcolor{Cyan!10!white}FORWARD-SYMGS  &       a[i] -= (val[i])[j]*b[(id[i])[j]]
	& 5 (3+1+1) & \hspace{0.35cm} 6.52
	\multirow{1}{*}{\begin{tikzpicture}[baseline=(current bounding box.east)]
		\draw [thick, red,decorate,decoration={brace,amplitude=10pt,mirror},rotate=90,xshift=-20pt,yshift=12pt](0,0) -- (1.15,0) node[black,midway,rotate=90,yshift=-0.6cm] {\footnotesize $\mathbf{10.17}$};	
		\end{tikzpicture}}
	 & 
	 \hspace{0.65cm} 40.2
	 \multirow{1}{*}{\begin{tikzpicture}[baseline=(current bounding box.east)]
	 	\draw [thick, red,decorate,decoration={brace,amplitude=10pt,mirror},rotate=90,xshift=-20pt,yshift=12pt](0,0) -- (1.15,0) node[black,midway,rotate=90,yshift=-0.6cm] {\footnotesize $\mathbf{39.9}$};	
	 	\end{tikzpicture}}
	  & 16.8 : 42.8    \\ 
	\cellcolor[gray]{0.9}& (+HALO-EXCHANGE)  &      a[i] += b[i]*diag[i][0]
	& 2 (2+0+0) & 8 &33.3 &  6 : 18  \\ 
	\cellcolor[gray]{0.9}&  &      b[i] = a[i]/diag[i][0]
	& 2 (0+1+1) & 16 & 46.2 &  6.87 : 14.87     \\
	\cellcolor[gray]{0.9}& \cellcolor{Cyan!10!white}BACKWARD-SYMGS  &       a[i] -= (val[i])[j]*b[(id[i])[j]]
	& 5 (3+1+1) & 6.52 & 40.2 & 16.8 : 42.8    \\ 
	&  &      a[i] += b[i]*diag[i][0]
	&2 (2+0+0) & 8 & 33.3 &  6 : 18 \\ 
	\multirow{-16}{*}{\rotatebox{90}{Multi Grid (MG) pre-conditioner}}&  &      b[i] = a[i]/diag[i][0]
	&2 (0+1+1) & 16 & 46.2 &  6.87 : 14.87   \\ 
		
	\specialrule{1.65pt}{0.15pt}{0.15pt}
	& \cellcolor{Cyan!10!white}DDOT2 & r += a[i]*b[i] & 2 (2+0+0) & 8 &33.3 & 6 : 18   \\ 
	\cellcolor[gray]{0.9}& (+ALLREDUCE) & & &   \\ \cline{2-7}
	\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white}DAXPY & c[i] = b[i] + r * c[i] & 3 (2+1+0) & 12 & 39.2 & 10.3 : 26.3   \\ \cline{2-7}
	\cellcolor[gray]{0.9}& \cellcolor{Cyan!10!white}SPMV  & t += (val[i])[j]*c[(id[i])[j]] & 5 (3+1+1) & 6.52 & 40.2 & 16.8 : 42.8    \\ 
	\cellcolor[gray]{0.9}& (+HALO-EXCHANGE)  & d[i] = t &  && &   \\ \cline{2-7}
	\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white}DDOT2 & r += c[i]*d[i] & 2 (2+0+0) & 8 & 33.3 & 6 : 18   \\ 
	\cellcolor[gray]{0.9}& (+ALLREDUCE) & & &   \\ \cline{2-7}
	\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white}DAXPY & e[i] = e[i] + r * c[i]  & 3 (2+1+0) & 12 &  39.2 & 10.3 : 26.3  \\ \cline{2-7}
	\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white}DAXPY & a[i] = a[i] - r * d[i]  & 3 (2+1+0) & 12 &  39.2 & 10.3 : 26.3  \\ \cline{2-7}
	\cellcolor[gray]{0.9}&\cellcolor{Cyan!10!white}DDOT1 & s += a[i]*a[i]  & 1 (1+0+0) & 4 & 33.3 & 3 :9   \\ 	
	\multirow{-11}{*}{\rotatebox{90}{Conjugate Gradient (CG)}}& (+ALLREDUCE) & & &   \\ 
	\specialrule{2.5pt}{1pt}{1pt}
	%\end{tabular}
\end{tabular*}
%SYMGS on Ivy Bridge:
%1: $T_{data}= (3*2)+(5*2)+(5*2)+(5*64*2.2/41.9) = 6+10+10+16.8=42.8$
%2: $T_{data}= (2*2)+(2*2)+(2*2)+(2*3) = 4+4+4+6=18$
%3: $T_{data}= (2*2)+(2*2)+(2*64*2.2/41) = 4+4+6.87=14.87$

%RESTRICTION on Ivy Bridge: 
%$T_{data}= (2.5*2)+(4.5*2)+(4.5*2)+(4.5*64*2.2/41.9)=5+9+9+15.12=38.12$ 

%PROLONGATION on Ivy Bridge:
%$T_{data}= (1*2)+(3.5*2)+(3.5*2)+(3.5*64*2.2/41) = 2+7+7+12=28$



==> tables/tab7_model.tex <==
\setlength\tabcolsep{3pt}
\setlength\extrarowheight{0pt} 
	\begin{tabular}[fragile]{llcc}
	\specialrule{2.5pt}{1pt}{1pt} 
	  
	\cellcolor[gray]{0.9}&
	\cellcolor{Cyan!12!white}$n_t^{\RN{1}}$   &
	IP&
	\cellcolor{Cyan!6!white}Number of threads on the NUMA domain for first kernel \\
	
	\cellcolor[gray]{0.9}&
	$n_t$  &IP&
	Total number of threads on the NUMA domain \\
	

	\cellcolor[gray]{0.9}&  
	\cellcolor{Cyan!12!white}$n_t-n_t^{\RN{1}}$ &IP&
	\cellcolor{Cyan!6!white}Number of threads on the NUMA domain for second kernel \\
	
	
	\cellcolor[gray]{0.9}	& ${b}_\mathrm{OL}(n_t)$&
	IP&
	 Achievable bandwidth (Weighted mean) of the architecture
	 \\

	\multirow{-5}{*}{\rotatebox{90}{\cellcolor[gray]{0.9}\textbf{Hybrid}}	} &  
	\cellcolor{Cyan!12!white}$b^{\RN{1}}_\mathrm{OL}(n_t,1)$  &OP&
	\cellcolor{Cyan!6!white}Per-core bandwidth share for first kernel \\
	
	\specialrule{.825pt}{0.075pt}{0.075pt}
	
	\cellcolor[gray]{0.9}&
	$T^{\RN{1}}$ &IP&
	Total time for first kernel\\
	
	\multirow{-2}{*}{\cellcolor[gray]{0.9}\rotatebox{90}{\textbf{Pure}}} &
	\cellcolor{Cyan!12!white}$\dfrac{n_\mathrm{CL}\cdot s_\mathrm{CL}}{b_s}$
%	$T^{\RN{1}}_\mathrm{L3-MEM}$ 
	&IP&
	\cellcolor{Cyan!6!white}Time contribution of first kernel for which memory bus is used\\
	
	\specialrule{2.5pt}{1pt}{1pt}
\end{tabular}

